On the Practicality of Deterministic Epistemic Uncertainty

A set of novel approaches for estimating epistemic uncertainty in deep neural networks with a single forward pass has recently emerged as a valid alternative to Bayesian Neural Networks. On the premise of informative representations, these deterministic uncertainty methods (DUMs) achieve strong performance on detecting out-of-distribution (OOD) data while adding negligible computational costs at inference time. However, it remains unclear whether DUMs are well calibrated and can seamlessly scale to real-world applications - both prerequisites for their practical deployment. To this end, we first provide a taxonomy of DUMs, and evaluate their calibration under continuous distributional shifts. Then, we extend them to semantic segmentation. We find that, while DUMs scale to realistic vision tasks and perform well on OOD detection, the practicality of current methods is undermined by poor calibration under distributional shifts.

==> figures/acc_vs_raulc/carla.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
title={CARLA-C},
x grid style={white!69.0196078431373!black},
xlabel={mIoU},
xmin=0.407, xmax=0.429,
xtick style={color=black},
xtick={0.405,0.41,0.415,0.42,0.425,0.43},
xticklabels={0.405,0.410,0.415,0.420,0.425,0.430},
y grid style={white!69.0196078431373!black},
ylabel={rAULC},
ymin=0, ymax=0.9,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
width=0.24\linewidth,
height=0.24\linewidth
]
\addplot [
  mark=x,
  only marks,
  scatter,
  scatter/@post marker code/.code={%
  \endscope
},
  scatter/@pre marker code/.code={%
  \expanded{%
  \noexpand\definecolor{thispointdrawcolor}{RGB}{\drawcolor}%
  \noexpand\definecolor{thispointfillcolor}{RGB}{\fillcolor}%
  }%
  \scope[draw=thispointdrawcolor, fill=thispointfillcolor]%
},
  visualization depends on={value \thisrow{draw} \as \drawcolor},
  visualization depends on={value \thisrow{fill} \as \fillcolor}
]
table{%
x  y  draw  fill
0.422 0.818 214,38.9999999999999,39.9999999999999 214,38.9999999999999,39.9999999999999
0.41 0.73 214,38.9999999999999,39.9999999999999 214,38.9999999999999,39.9999999999999
0.428 0.812 214,38.9999999999999,39.9999999999999 214,38.9999999999999,39.9999999999999
0.424 0.813 30.9999999999999,119,180 30.9999999999999,119,180
0.408 0.002 30.9999999999999,119,180 30.9999999999999,119,180
0.412 0.619 30.9999999999999,119,180 30.9999999999999,119,180
};
\draw (axis cs:0.421881535247312,0.823375413907285) node[
  scale=0.5,
  anchor=south east,
  text=black,
  rotate=0.0
]{Softmax};
\draw (axis cs:0.410045216387097,0.735215231788079) node[
  scale=0.5,
  anchor=south west,
  text=black,
  rotate=0.0
]{MCD};
\draw (axis cs:0.428183571236559,0.80312417218543) node[
  scale=0.5,
  anchor=north east,
  text=black,
  rotate=0.0
]{Ensemble};
\draw (axis cs:0.424053421677419,0.818215231788079) node[
  scale=0.5,
  anchor=south west,
  text=black,
  rotate=0.0
]{SNGP};
\draw (axis cs:0.408043994322581,0.00743791390728475) node[
  scale=0.5,
  anchor=south west,
  text=black,
  rotate=0.0
]{DDU};
\draw (axis cs:0.412035963612903,0.624215231788079) node[
  scale=0.5,
  anchor=south west,
  text=black,
  rotate=0.0
]{MIR};
\end{axis}

\end{tikzpicture}


==> figures/acc_vs_raulc/cifar10.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
title={CIFAR10-C},
x grid style={white!69.0196078431373!black},
xlabel={Accuracy},
xmin=0.85575, xmax=0.94925,
xtick style={color=black},
xtick={0.84,0.88,0.92,0.96},
xticklabels={0.84,0.88,0.92,0.96},
y grid style={white!69.0196078431373!black},
ylabel={rAULC},
ymin=0.4214, ymax=0.8526,
ytick style={color=black},
ytick={0.4,0.5,0.6,0.7,0.8,0.9},
yticklabels={0.4,0.5,0.6,0.7,0.8,0.9},
width=0.24\linewidth,
height=0.24\linewidth
]
\addplot [
  mark=*,
  mark size=0.04,
  only marks,
  scatter,
  scatter/@post marker code/.code={%
  \endscope
},
  scatter/@pre marker code/.code={%
  \expanded{%
  \noexpand\definecolor{thispointdrawcolor}{RGB}{\drawcolor}%
  \noexpand\definecolor{thispointfillcolor}{RGB}{\fillcolor}%
  }%
  \scope[draw=thispointdrawcolor, fill=thispointfillcolor]%
},
  visualization depends on={value \thisrow{draw} \as \drawcolor},
  visualization depends on={value \thisrow{fill} \as \fillcolor}
]
table{%
x  y  draw  fill
0.882 0.708 214,38.9999999999999,39.9999999999999 214,38.9999999999999,39.9999999999999
0.885 0.829 214,38.9999999999999,39.9999999999999 214,38.9999999999999,39.9999999999999
0.91 0.833 214,38.9999999999999,39.9999999999999 214,38.9999999999999,39.9999999999999
0.903 0.766 30.9999999999999,119,180 30.9999999999999,119,180
0.884 0.441 30.9999999999999,119,180 30.9999999999999,119,180
0.889 0.697 30.9999999999999,119,180 30.9999999999999,119,180
0.86 0.614 30.9999999999999,119,180 30.9999999999999,119,180
0.945 0.706 30.9999999999999,119,180 30.9999999999999,119,180
};
\draw (axis cs:0.882514176044516,0.711092110927152) node[
  scale=0.8,
  anchor=south west,
  text=black,
  rotate=0.0
]{Softmax};
\draw (axis cs:0.88528838367871,0.825907889072848) node[
  scale=0.8,
  anchor=north west,
  text=black,
  rotate=0.0
]{MCD};
\draw (axis cs:0.910607367554839,0.829907889072848) node[
  scale=0.8,
  anchor=north west,
  text=black,
  rotate=0.0
]{Ensemble};
\draw (axis cs:0.903342165843871,0.766) node[
  scale=0.8,
  anchor=west,
  text=black,
  rotate=0.0
]{SNGP};
\draw (axis cs:0.884281429088387,0.444092110927152) node[
  scale=0.8,
  anchor=south west,
  text=black,
  rotate=0.0
]{DDU};
\draw (axis cs:0.88922903784129,0.693907889072848) node[
  scale=0.8,
  anchor=north west,
  text=black,
  rotate=0.0
]{MIR};
\draw (axis cs:0.860283283645806,0.617092110927152) node[
  scale=0.8,
  anchor=south west,
  text=black,
  rotate=0.0
]{DUQ};
\draw (axis cs:0.94472784369871,0.709092110927152) node[
  scale=0.8,
  anchor=south east,
  text=black,
  rotate=0.0
]{DCU};
\end{axis}

\end{tikzpicture}


==> figures/acc_vs_raulc/cifar100.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
title={CIFAR100-C},
x grid style={white!69.0196078431373!black},
xlabel={Accuracy},
xmin=0.60735, xmax=0.64365,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={rAULC},
ymin=0.31965, ymax=0.74535,
ytick style={color=black},
ytick={0.3,0.4,0.5,0.6,0.7,0.8},
yticklabels={0.3,0.4,0.5,0.6,0.7,0.8},
width=0.24\linewidth,
height=0.24\linewidth
]
\addplot [
  mark=x,
  only marks,
  scatter,
  scatter/@post marker code/.code={%
  \endscope
},
  scatter/@pre marker code/.code={%
  \expanded{%
  \noexpand\definecolor{thispointdrawcolor}{RGB}{\drawcolor}%
  \noexpand\definecolor{thispointfillcolor}{RGB}{\fillcolor}%
  }%
  \scope[draw=thispointdrawcolor, fill=thispointfillcolor]%
},
  visualization depends on={value \thisrow{draw} \as \drawcolor},
  visualization depends on={value \thisrow{fill} \as \fillcolor}
]
table{%
x  y  draw  fill
0.61 0.596 214,38.9999999999999,39.9999999999999 214,38.9999999999999,39.9999999999999
0.615 0.726 214,38.9999999999999,39.9999999999999 214,38.9999999999999,39.9999999999999
0.628 0.713 214,38.9999999999999,39.9999999999999 214,38.9999999999999,39.9999999999999
0.611 0.623 30.9999999999999,119,180 30.9999999999999,119,180
0.609 0.339 30.9999999999999,119,180 30.9999999999999,119,180
0.617 0.514 30.9999999999999,119,180 30.9999999999999,119,180
0.642 0.558 30.9999999999999,119,180 30.9999999999999,119,180
};
\draw (axis cs:0.610165781069548,0.59340985513245) node[
  scale=0.5,
  anchor=north west,
  text=black,
  rotate=0.0
]{Softmax};
\draw (axis cs:0.615093240601548,0.72340985513245) node[
  scale=0.5,
  anchor=north west,
  text=black,
  rotate=0.0
]{MCD};
\draw (axis cs:0.628196201265806,0.71559014486755) node[
  scale=0.5,
  anchor=south west,
  text=black,
  rotate=0.0
]{Ensemble};
\draw (axis cs:0.61111016071071,0.62559014486755) node[
  scale=0.5,
  anchor=south west,
  text=black,
  rotate=0.0
]{SNGP};
\draw (axis cs:0.60909072058529,0.34159014486755) node[
  scale=0.5,
  anchor=south west,
  text=black,
  rotate=0.0
]{DDU};
\draw (axis cs:0.617074160478452,0.51659014486755) node[
  scale=0.5,
  anchor=south west,
  text=black,
  rotate=0.0
]{MIR};
\draw (axis cs:0.64191215943329,0.56059014486755) node[
  scale=0.5,
  anchor=south east,
  text=black,
  rotate=0.0
]{DCU};
\end{axis}

\end{tikzpicture}


==> figures/acc_vs_raulc/cityscape.tex <==
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
title={Cityscape-C},
x grid style={white!69.0196078431373!black},
xlabel={mIoU},
xmin=0.5019, xmax=0.5261,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={rAULC},
ymin=0, ymax=0.9,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
width=0.24\linewidth,
height=0.24\linewidth
]
\addplot [
  mark=x,
  only marks,
  scatter,
  scatter/@post marker code/.code={%
  \endscope
},
  scatter/@pre marker code/.code={%
  \expanded{%
  \noexpand\definecolor{thispointdrawcolor}{RGB}{\drawcolor}%
  \noexpand\definecolor{thispointfillcolor}{RGB}{\fillcolor}%
  }%
  \scope[draw=thispointdrawcolor, fill=thispointfillcolor]%
},
  visualization depends on={value \thisrow{draw} \as \drawcolor},
  visualization depends on={value \thisrow{fill} \as \fillcolor}
]
table{%
x  y  draw  fill
0.503 0.737 214,38.9999999999999,39.9999999999999 214,38.9999999999999,39.9999999999999
0.506 0.785 214,38.9999999999999,39.9999999999999 214,38.9999999999999,39.9999999999999
0.525 0.751 214,38.9999999999999,39.9999999999999 214,38.9999999999999,39.9999999999999
0.519 0.759 30.9999999999999,119,180 30.9999999999999,119,180
0.505 0.542 30.9999999999999,119,180 30.9999999999999,119,180
0.504 0.564 30.9999999999999,119,180 30.9999999999999,119,180
};
\draw (axis cs:0.503110520713032,0.731524006622516) node[
  scale=0.5,
  anchor=north west,
  text=black,
  rotate=0.0
]{Softmax};
\draw (axis cs:0.506062160401032,0.790475993377483) node[
  scale=0.5,
  anchor=south west,
  text=black,
  rotate=0.0
]{MCD};
\draw (axis cs:0.524914014769376,0.745499586092715) node[
  scale=0.5,
  anchor=north east,
  text=black,
  rotate=0.0
]{Ensemble};
\draw (axis cs:0.518843327150538,0.762562913907285) node[
  scale=0.5,
  anchor=south east,
  text=black,
  rotate=0.0
]{SNGP};
\draw (axis cs:0.505060480390193,0.536524006622517) node[
  scale=0.5,
  anchor=north west,
  text=black,
  rotate=0.0
]{DDU};
\draw (axis cs:0.504049440318968,0.569475993377483) node[
  scale=0.5,
  anchor=south west,
  text=black,
  rotate=0.0
]{MIR};
\end{axis}

\end{tikzpicture}


==> figures/cifar_10_100_c_main/gaussian_cifar10.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color1}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}
\definecolor{color2}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color3}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color4}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color5}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color6}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}
\definecolor{color7}{rgb}{0.0901960784313725,0.745098039215686,0.811764705882353}

\begin{groupplot}[group style={group size=3 by 1, horizontal sep=0.04\linewidth}]
\nextgroupplot[
legend cell align={left},
yticklabel style={rotate=90},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
title={Accuracy - gn},
x grid style={white!69.0196078431373!black},
xmin=-0.25, xmax=5.25,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0.07875, ymax=0.98625,
ytick style={color=black},
width=0.23\linewidth,
height=0.23\linewidth,
ytick={0.4, 0.8},
tick label style={font=\tiny},
]
\addplot [semithick, color0]
table {%
0 0.903
1 0.713
2 0.497
3 0.319
4 0.259
5 0.217
};
% \addlegendentry{sngp}
\addplot [semithick, color1]
table {%
0 0.884
1 0.761
2 0.605
3 0.434
4 0.362
5 0.301
};
% \addlegendentry{ddu}
\addplot [semithick, color2]
table {%
0 0.889
1 0.767
2 0.616
3 0.458
4 0.385
5 0.328
};
% \addlegendentry{mir}
\addplot [semithick, color3]
table {%
0 0.86
1 0.678
2 0.481
3 0.313
4 0.254
5 0.214
};
% \addlegendentry{duq}
\addplot [semithick, color4]
table {%
0 0.879
1 0.746
2 0.576
3 0.402
4 0.328
5 0.27
};
% \addlegendentry{softmax}
\addplot [semithick, color5]
table {%
0 0.916
1 0.801
2 0.636
3 0.45
4 0.371
5 0.303
};
% \addlegendentry{ensemble}
\addplot [semithick, color6]
table {%
0 0.885
1 0.803
2 0.638
3 0.452
4 0.373
5 0.305
};
% \addlegendentry{dropout}
\addplot [semithick, color7]
table {%
0 0.945
1 0.568
2 0.347
3 0.207
4 0.151
5 0.12
};
% \addlegendentry{winkens}

\nextgroupplot[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(-0.0,1.7)},
  anchor=north west,
  draw=white,
  legend columns=4,
  legend image post style={scale=0.25},
},
tick align=outside,
yticklabel style={rotate=90},
tick pos=left,
title={AUROC - gn},
x grid style={white!69.0196078431373!black},
xmin=-0.25, xmax=5.25,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0.4772, ymax=0.9348,
ytick style={color=black},
width=0.23\linewidth,
height=0.23\linewidth,
tick label style={font=\tiny},
]
\addplot [semithick, color0]
table {%
0 0.889
1 0.824
2 0.739
3 0.67
4 0.641
5 0.631
};
\addlegendentry{SNGP}
\addplot [semithick, color1]
table {%
0 0.751
1 0.668
2 0.58
3 0.523
4 0.501
5 0.498
};
\addlegendentry{DDU}
\addplot [semithick, color2]
table {%
0 0.849
1 0.773
2 0.688
3 0.618
4 0.599
5 0.585
};
\addlegendentry{MIR}
\addplot [semithick, color3]
table {%
0 0.854
1 0.763
2 0.666
3 0.585
4 0.559
5 0.549
};
\addlegendentry{DUQ}
\addplot [semithick, color4]
table {%
0 0.905
1 0.849
2 0.774
3 0.696
4 0.658
5 0.638
};
%\addlegendentry{Softmax}
\addplot [semithick, color5]
table {%
0 0.914
1 0.864
2 0.787
3 0.704
4 0.666
5 0.645
};
%\addlegendentry{Ensemble}
\addplot [semithick, color6]
table {%
0 0.899
1 0.866
2 0.789
3 0.706
4 0.668
5 0.647
};
%\addlegendentry{MC Dropout}
\addplot [semithick, color7]
table {%
0 0.849
1 0.643
2 0.616
3 0.61
4 0.61
5 0.602
};
%\addlegendentry{DCU}

\nextgroupplot[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
title={rAULC - gn},
yticklabel style={rotate=90},
x grid style={white!69.0196078431373!black},
xmin=-0.25, xmax=5.25,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0.00849999999999999, ymax=0.9435,
ytick style={color=black},
width=0.23\linewidth,
height=0.23\linewidth,
ytick={0.4, 0.8},
tick label style={font=\tiny},
]
\addplot [semithick, color0]
table {%
0 0.856
1 0.758
2 0.581
3 0.422
4 0.36
5 0.329
};
% \addlegendentry{sngp}
\addplot [semithick, color1]
table {%
0 0.626
1 0.422
2 0.21
3 0.091
4 0.062
5 0.051
};
% \addlegendentry{ddu}
\addplot [semithick, color2]
table {%
0 0.802
1 0.667
2 0.487
3 0.341
4 0.302
5 0.273
};
% \addlegendentry{mir}
\addplot [semithick, color3]
table {%
0 0.777
1 0.6
2 0.369
3 0.185
4 0.13
5 0.105
};
% \addlegendentry{duq}
\addplot [semithick, color4]
table {%
0 0.887
1 0.803
2 0.663
3 0.493
4 0.411
5 0.364
};
% \addlegendentry{softmax}
\addplot [semithick, color5]
table {%
0 0.901
1 0.828
2 0.69
3 0.514
4 0.433
5 0.388
};
% \addlegendentry{ensemble}
\addplot [semithick, color6]
table {%
0 0.879
1 0.83
2 0.692
3 0.516
4 0.435
5 0.39
};
% \addlegendentry{dropout}
\addplot [semithick, color7]
table {%
0 0.808
1 0.444
2 0.347
3 0.273
4 0.18
5 0.132
};
% \addlegendentry{winkens}
\end{groupplot}

\end{tikzpicture}


==> figures/cifar_10_100_c_main/gaussian_cifar100.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color1}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}
\definecolor{color2}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color3}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}
\definecolor{color6}{rgb}{0.0901960784313725,0.745098039215686,0.811764705882353}

\begin{groupplot}[group style={group size=3 by 1, horizontal sep=0.04\linewidth}]
\nextgroupplot[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.25, xmax=5.25,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0.07875, ymax=0.98625,
ytick style={color=black},
width=0.23\linewidth,
height=0.23\linewidth,
xlabel={Severity},
yticklabel style={rotate=90},
ytick={0.4, 0.8},
tick label style={font=\tiny}  
]
\addplot [semithick, color0]
table {%
0 0.903
1 0.713
2 0.497
3 0.319
4 0.259
5 0.217
};
% \addlegendentry{sngp}
\addplot [semithick, color1]
table {%
0 0.884
1 0.761
2 0.605
3 0.434
4 0.362
5 0.301
};
% \addlegendentry{ddu}
\addplot [semithick, color2]
table {%
0 0.889
1 0.767
2 0.616
3 0.458
4 0.385
5 0.328
};
% \addlegendentry{mir}
\addplot [semithick, color3]
table {%
0 0.879
1 0.746
2 0.576
3 0.402
4 0.328
5 0.27
};
% \addlegendentry{softmax}
\addplot [semithick, color4]
table {%
0 0.916
1 0.801
2 0.636
3 0.45
4 0.371
5 0.303
};
% \addlegendentry{ensemble}
\addplot [semithick, color5]
table {%
0 0.885
1 0.803
2 0.638
3 0.452
4 0.373
5 0.305
};
% \addlegendentry{dropout}
\addplot [semithick, color6]
table {%
0 0.945
1 0.568
2 0.347
3 0.207
4 0.151
5 0.12
};
% \addlegendentry{winkens}

\nextgroupplot[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
yticklabel style={rotate=90},
xmin=-0.25, xmax=5.25,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0.4772, ymax=0.9348,
ytick style={color=black},
width=0.23\linewidth,
height=0.23\linewidth,
xlabel={Severity},
ytick={0.6, 0.8},
tick label style={font=\tiny}  
]
\addplot [semithick, color0]
table {%
0 0.889
1 0.824
2 0.739
3 0.67
4 0.641
5 0.631
};
% \addlegendentry{sngp}
\addplot [semithick, color1]
table {%
0 0.751
1 0.668
2 0.58
3 0.523
4 0.501
5 0.498
};
% \addlegendentry{ddu}
\addplot [semithick, color2]
table {%
0 0.849
1 0.773
2 0.688
3 0.618
4 0.599
5 0.585
};
% \addlegendentry{mir}
\addplot [semithick, color3]
table {%
0 0.905
1 0.849
2 0.774
3 0.696
4 0.658
5 0.638
};
% \addlegendentry{softmax}
\addplot [semithick, color4]
table {%
0 0.914
1 0.864
2 0.787
3 0.704
4 0.666
5 0.645
};
% \addlegendentry{ensemble}
\addplot [semithick, color5]
table {%
0 0.899
1 0.866
2 0.789
3 0.706
4 0.668
5 0.647
};
% \addlegendentry{dropout}
\addplot [semithick, color6]
table {%
0 0.849
1 0.643
2 0.616
3 0.61
4 0.61
5 0.602
};
% \addlegendentry{winkens}

\nextgroupplot[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
yticklabel style={rotate=90},
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.25, xmax=5.25,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0.00849999999999999, ymax=0.9435,
ytick style={color=black},
width=0.23\linewidth,
height=0.23\linewidth,
xlabel={Severity},
ytick={0.4, 0.8},
tick label style={font=\tiny}  
]
\addplot [semithick, color0]
table {%
0 0.856
1 0.758
2 0.581
3 0.422
4 0.36
5 0.329
};
% \addlegendentry{sngp}
\addplot [semithick, color1]
table {%
0 0.626
1 0.422
2 0.21
3 0.091
4 0.062
5 0.051
};
% \addlegendentry{ddu}
\addplot [semithick, color2]
table {%
0 0.802
1 0.667
2 0.487
3 0.341
4 0.302
5 0.273
};
% \addlegendentry{mir}
\addplot [semithick, color3]
table {%
0 0.887
1 0.803
2 0.663
3 0.493
4 0.411
5 0.364
};
% \addlegendentry{softmax}
\addplot [semithick, color4]
table {%
0 0.901
1 0.828
2 0.69
3 0.514
4 0.433
5 0.388
};
% \addlegendentry{ensemble}
\addplot [semithick, color5]
table {%
0 0.879
1 0.83
2 0.692
3 0.516
4 0.435
5 0.39
};
% \addlegendentry{dropout}
\addplot [semithick, color6]
table {%
0 0.808
1 0.444
2 0.347
3 0.273
4 0.18
5 0.132
};
% \addlegendentry{winkens}
\end{groupplot}

\end{tikzpicture}


==> figures/cifar_10_100_c_main/motion_blur_cifar10.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color1}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}
\definecolor{color2}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color3}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color4}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color5}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color6}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}
\definecolor{color7}{rgb}{0.0901960784313725,0.745098039215686,0.811764705882353}



\begin{groupplot}[group style={group size=3 by 1, horizontal sep=0.04\linewidth}]
\nextgroupplot[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
title={Accuracy - mb},
x grid style={white!69.0196078431373!black},
xmin=-0.25, xmax=5.25,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0.2184, ymax=0.9796,
ytick style={color=black},
width=0.23\linewidth,
height=0.23\linewidth,
yticklabel style={rotate=90},
ytick={0.4, 0.8},
tick label style={font=\tiny},
]
\addplot [semithick, color0]
table {%
0 0.903
1 0.826
2 0.719
3 0.604
4 0.606
5 0.51
};
% \addlegendentry{sngp}
\addplot [semithick, color1]
table {%
0 0.884
1 0.813
2 0.721
3 0.624
4 0.623
5 0.542
};
% \addlegendentry{ddu}
\addplot [semithick, color2]
table {%
0 0.889
1 0.814
2 0.722
3 0.623
4 0.621
5 0.534
};
% \addlegendentry{mir}
\addplot [semithick, color3]
table {%
0 0.86
1 0.778
2 0.669
3 0.568
4 0.564
5 0.48
};
% \addlegendentry{duq}
\addplot [semithick, color4]
table {%
0 0.879
1 0.809
2 0.713
3 0.615
4 0.614
5 0.525
};
% \addlegendentry{softmax}
\addplot [semithick, color5]
table {%
0 0.916
1 0.861
2 0.775
3 0.678
4 0.678
5 0.585
};
% \addlegendentry{ensemble}
\addplot [semithick, color6]
table {%
0 0.885
1 0.821
2 0.735
3 0.638
4 0.638
5 0.545
};
% \addlegendentry{dropout}
\addplot [semithick, color7]
table {%
0 0.945
1 0.703
2 0.481
3 0.337
4 0.27
5 0.253
};
% \addlegendentry{winkens}

\nextgroupplot[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(-1.93,1.7)},
  anchor=north west,
  draw=white,
  legend columns=4,
  legend image post style={scale=0.25},
},
tick align=outside,
tick pos=left,
title={AUROC - mb},
x grid style={white!69.0196078431373!black},
xmin=-0.25, xmax=5.25,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0.5843, ymax=0.9297,
ytick style={color=black},
width=0.23\linewidth,
height=0.23\linewidth,
yticklabel style={rotate=90},
ytick={0.6, 0.8},
tick label style={font=\tiny},
]

\addplot [semithick, color4]
table {%
0 0.905
1 0.872
2 0.834
3 0.791
4 0.792
5 0.759
};
\addlegendentry{Softmax}
\addplot [semithick, color5]
table {%
0 0.914
1 0.881
2 0.845
3 0.801
4 0.805
5 0.777
};
\addlegendentry{Ensemble}
\addplot [semithick, color6]
table {%
0 0.899
1 0.841
2 0.805
3 0.761
4 0.765
5 0.737
};
\addlegendentry{MC Dropout}
\addplot [semithick, color7]
table {%
0 0.849
1 0.63
2 0.6
3 0.614
4 0.615
5 0.617
};
\addlegendentry{DCU}


\addplot [semithick, color0]
table {%
0 0.889
1 0.859
2 0.814
3 0.775
4 0.775
5 0.738
};
%\addlegendentry{sngp}
\addplot [semithick, color1]
table {%
0 0.751
1 0.71
2 0.667
3 0.632
4 0.641
5 0.618
};
%\addlegendentry{ddu}
\addplot [semithick, color2]
table {%
0 0.849
1 0.807
2 0.763
3 0.728
4 0.728
5 0.704
};
%\addlegendentry{mir}
\addplot [semithick, color3]
table {%
0 0.854
1 0.835
2 0.8
3 0.757
4 0.758
5 0.724
};
%\addlegendentry{duq}


\nextgroupplot[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
title={rAULC - mb},
x grid style={white!69.0196078431373!black},
xmin=-0.25, xmax=5.25,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0.2626, ymax=0.9314,
ytick style={color=black},
width=0.23\linewidth,
height=0.23\linewidth,
yticklabel style={rotate=90},
ytick={0.4, 0.8},
tick label style={font=\tiny},
]
\addplot [semithick, color0]
table {%
0 0.856
1 0.819
2 0.746
3 0.67
4 0.672
5 0.592
};
% \addlegendentry{sngp}
\addplot [semithick, color1]
table {%
0 0.626
1 0.556
2 0.468
3 0.389
4 0.407
5 0.354
};
% \addlegendentry{ddu}
\addplot [semithick, color2]
table {%
0 0.802
1 0.74
2 0.666
3 0.593
4 0.595
5 0.539
};
% \addlegendentry{mir}
\addplot [semithick, color3]
table {%
0 0.777
1 0.754
2 0.694
3 0.604
4 0.606
5 0.53
};
% \addlegendentry{duq}
\addplot [semithick, color4]
table {%
0 0.887
1 0.84
2 0.779
3 0.702
4 0.703
5 0.633
};
% \addlegendentry{softmax}
\addplot [semithick, color5]
table {%
0 0.901
1 0.856
2 0.8
3 0.725
4 0.729
5 0.67
};
% \addlegendentry{ensemble}
\addplot [semithick, color6]
table {%
0 0.879
1 0.816
2 0.76
3 0.685
4 0.689
5 0.63
};
% \addlegendentry{dropout}
\addplot [semithick, color7]
table {%
0 0.808
1 0.404
2 0.317
3 0.302
4 0.293
5 0.294
};
% \addlegendentry{winkens}
\end{groupplot}

\end{tikzpicture}


==> figures/cifar_10_100_c_main/motion_blur_cifar100.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color1}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}
\definecolor{color2}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color3}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}
\definecolor{color6}{rgb}{0.0901960784313725,0.745098039215686,0.811764705882353}

\begin{groupplot}[group style={group size=3 by 1, horizontal sep=0.04\linewidth}]
\nextgroupplot[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.25, xmax=5.25,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0.2184, ymax=0.9796,
ytick style={color=black},
width=0.23\linewidth,
height=0.23\linewidth,
xlabel={Severity},
yticklabel style={rotate=90},
ytick={0.4, 0.8},
tick label style={font=\tiny}  
]
\addplot [semithick, color0]
table {%
0 0.903
1 0.826
2 0.719
3 0.604
4 0.606
5 0.51
};
% \addlegendentry{sngp}
\addplot [semithick, color1]
table {%
0 0.884
1 0.813
2 0.721
3 0.624
4 0.623
5 0.542
};
% \addlegendentry{ddu}
\addplot [semithick, color2]
table {%
0 0.889
1 0.814
2 0.722
3 0.623
4 0.621
5 0.534
};
% \addlegendentry{mir}
\addplot [semithick, color3]
table {%
0 0.879
1 0.809
2 0.713
3 0.615
4 0.614
5 0.525
};
% \addlegendentry{softmax}
\addplot [semithick, color4]
table {%
0 0.916
1 0.861
2 0.775
3 0.678
4 0.678
5 0.585
};
% \addlegendentry{ensemble}
\addplot [semithick, color5]
table {%
0 0.885
1 0.821
2 0.735
3 0.638
4 0.638
5 0.545
};
% \addlegendentry{dropout}
\addplot [semithick, color6]
table {%
0 0.945
1 0.703
2 0.481
3 0.337
4 0.27
5 0.253
};
% \addlegendentry{winkens}

\nextgroupplot[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.25, xmax=5.25,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0.5843, ymax=0.9297,
ytick style={color=black},
width=0.23\linewidth,
height=0.23\linewidth,
xlabel={Severity},
yticklabel style={rotate=90},
ytick={0.7, 0.8},
tick label style={font=\tiny}  
]
\addplot [semithick, color0]
table {%
0 0.889
1 0.859
2 0.814
3 0.775
4 0.775
5 0.738
};
% \addlegendentry{sngp}
\addplot [semithick, color1]
table {%
0 0.751
1 0.71
2 0.667
3 0.632
4 0.641
5 0.618
};
% \addlegendentry{ddu}
\addplot [semithick, color2]
table {%
0 0.849
1 0.807
2 0.763
3 0.728
4 0.728
5 0.704
};
% \addlegendentry{mir}
\addplot [semithick, color3]
table {%
0 0.905
1 0.872
2 0.834
3 0.791
4 0.792
5 0.759
};
% \addlegendentry{softmax}
\addplot [semithick, color4]
table {%
0 0.914
1 0.881
2 0.845
3 0.801
4 0.805
5 0.777
};
% \addlegendentry{ensemble}
\addplot [semithick, color5]
table {%
0 0.899
1 0.841
2 0.805
3 0.761
4 0.765
5 0.737
};
% \addlegendentry{dropout}
\addplot [semithick, color6]
table {%
0 0.849
1 0.63
2 0.6
3 0.614
4 0.615
5 0.617
};
% \addlegendentry{winkens}

\nextgroupplot[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.25, xmax=5.25,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0.2626, ymax=0.9314,
ytick style={color=black},
width=0.23\linewidth,
height=0.23\linewidth,
xlabel={Severity},
yticklabel style={rotate=90},
ytick={0.4, 0.8},
tick label style={font=\tiny}  
]
\addplot [semithick, color0]
table {%
0 0.856
1 0.819
2 0.746
3 0.67
4 0.672
5 0.592
};
% \addlegendentry{sngp}
\addplot [semithick, color1]
table {%
0 0.626
1 0.556
2 0.468
3 0.389
4 0.407
5 0.354
};
% \addlegendentry{ddu}
\addplot [semithick, color2]
table {%
0 0.802
1 0.74
2 0.666
3 0.593
4 0.595
5 0.539
};
% \addlegendentry{mir}
\addplot [semithick, color3]
table {%
0 0.887
1 0.84
2 0.779
3 0.702
4 0.703
5 0.633
};
% \addlegendentry{softmax}
\addplot [semithick, color4]
table {%
0 0.901
1 0.856
2 0.8
3 0.725
4 0.729
5 0.67
};
% \addlegendentry{ensemble}
\addplot [semithick, color5]
table {%
0 0.879
1 0.816
2 0.76
3 0.685
4 0.689
5 0.63
};
% \addlegendentry{dropout}
\addplot [semithick, color6]
table {%
0 0.808
1 0.404
2 0.317
3 0.302
4 0.293
5 0.294
};
% \addlegendentry{winkens}
\end{groupplot}

\end{tikzpicture}


==> figures/cityscapes_c_main/gaussian_noise.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color2}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color3}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}
\definecolor{color4}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color5}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
title={mIoU},
xmajorticks=false,
ymin=-0.018, ymax=0.554,
corrupted cityscapes plots,
]
\path [draw=color0, fill=color0, opacity=0.2]
(axis cs:0,0.52)
--(axis cs:0,0.484)
--(axis cs:1,0.132)
--(axis cs:2,0.037)
--(axis cs:3,0.023)
--(axis cs:4,0.018)
--(axis cs:5,0.016)
--(axis cs:5,0.04)
--(axis cs:5,0.04)
--(axis cs:4,0.048)
--(axis cs:3,0.051)
--(axis cs:2,0.101)
--(axis cs:1,0.196)
--(axis cs:0,0.52)
--cycle;

\path [draw=color1, fill=color1, opacity=0.2]
(axis cs:0,0.528)
--(axis cs:0,0.522)
--(axis cs:1,0.163)
--(axis cs:2,0.047)
--(axis cs:3,0.014)
--(axis cs:4,0.015)
--(axis cs:5,0.018)
--(axis cs:5,0.024)
--(axis cs:5,0.024)
--(axis cs:4,0.027)
--(axis cs:3,0.028)
--(axis cs:2,0.097)
--(axis cs:1,0.225)
--(axis cs:0,0.528)
--cycle;

\path [draw=color2, fill=color2, opacity=0.2]
(axis cs:0,0.528)
--(axis cs:0,0.51)
--(axis cs:1,0.126)
--(axis cs:2,0.033)
--(axis cs:3,0.017)
--(axis cs:4,0.013)
--(axis cs:5,0.01)
--(axis cs:5,0.028)
--(axis cs:5,0.028)
--(axis cs:4,0.031)
--(axis cs:3,0.039)
--(axis cs:2,0.077)
--(axis cs:1,0.19)
--(axis cs:0,0.528)
--cycle;

\path [draw=color3, fill=color3, opacity=0.2]
(axis cs:0,0.514)
--(axis cs:0,0.498)
--(axis cs:1,0.366)
--(axis cs:2,0.298)
--(axis cs:3,0.199)
--(axis cs:4,0.157)
--(axis cs:5,0.115)
--(axis cs:5,0.165)
--(axis cs:5,0.165)
--(axis cs:4,0.215)
--(axis cs:3,0.251)
--(axis cs:2,0.328)
--(axis cs:1,0.384)
--(axis cs:0,0.514)
--cycle;

\path [draw=color4, fill=color4, opacity=0.2]
(axis cs:0,0.517)
--(axis cs:0,0.491)
--(axis cs:1,0.12)
--(axis cs:2,0.032)
--(axis cs:3,0.026)
--(axis cs:4,0.025)
--(axis cs:5,0.019)
--(axis cs:5,0.027)
--(axis cs:5,0.027)
--(axis cs:4,0.039)
--(axis cs:3,0.07)
--(axis cs:2,0.146)
--(axis cs:1,0.234)
--(axis cs:0,0.517)
--cycle;

\path [draw=color5, fill=color5, opacity=0.2]
(axis cs:0,0.519)
--(axis cs:0,0.491)
--(axis cs:1,0.052)
--(axis cs:2,0.019)
--(axis cs:3,0.02)
--(axis cs:4,0.013)
--(axis cs:5,0.008)
--(axis cs:5,0.026)
--(axis cs:5,0.026)
--(axis cs:4,0.033)
--(axis cs:3,0.028)
--(axis cs:2,0.035)
--(axis cs:1,0.1)
--(axis cs:0,0.519)
--cycle;

\addplot [semithick, color0]
table {%
0 0.502
1 0.164
2 0.069
3 0.037
4 0.033
5 0.028
};
%\addlegendentry{softmax}
\addplot [semithick, color1]
table {%
0 0.525
1 0.194
2 0.072
3 0.021
4 0.021
5 0.021
};
%\addlegendentry{ensemble}
\addplot [semithick, color2]
table {%
0 0.519
1 0.158
2 0.055
3 0.028
4 0.022
5 0.019
};
%\addlegendentry{sngp}
\addplot [semithick, color3]
table {%
0 0.506
1 0.375
2 0.313
3 0.225
4 0.186
5 0.14
};
%\addlegendentry{dropout}
\addplot [semithick, color4]
table {%
0 0.504
1 0.177
2 0.089
3 0.048
4 0.032
5 0.023
};
%\addlegendentry{mir}
\addplot [semithick, color5]
table {%
0 0.505
1 0.076
2 0.027
3 0.024
4 0.023
5 0.017
};
%\addlegendentry{ddu}

\nextgroupplot[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(-0.35,1.50)},
  anchor=north west,
  draw=white,
  legend columns=6,
  legend image post style={scale=0.45},
},
title={AUROC},
xmajorticks=false,
ymin=0.33095, ymax=0.92605, 
corrupted cityscapes plots, 
]
\path [draw=color0, fill=color0, opacity=0.2]
(axis cs:0,0.899)
--(axis cs:0,0.891)
--(axis cs:1,0.576)
--(axis cs:2,0.493)
--(axis cs:3,0.505)
--(axis cs:4,0.508)
--(axis cs:5,0.498)
--(axis cs:5,0.624)
--(axis cs:5,0.624)
--(axis cs:4,0.65)
--(axis cs:3,0.653)
--(axis cs:2,0.681)
--(axis cs:1,0.696)
--(axis cs:0,0.899)
--cycle;

\path [draw=color1, fill=color1, opacity=0.2]
(axis cs:0,0.873)
--(axis cs:0,0.871)
--(axis cs:1,0.655)
--(axis cs:2,0.501)
--(axis cs:3,0.588)
--(axis cs:4,0.605)
--(axis cs:5,0.556)
--(axis cs:5,0.674)
--(axis cs:5,0.674)
--(axis cs:4,0.699)
--(axis cs:3,0.66)
--(axis cs:2,0.619)
--(axis cs:1,0.677)
--(axis cs:0,0.873)
--cycle;

\path [draw=color2, fill=color2, opacity=0.2]
(axis cs:0,0.87)
--(axis cs:0,0.86)
--(axis cs:1,0.645)
--(axis cs:2,0.565)
--(axis cs:3,0.556)
--(axis cs:4,0.558)
--(axis cs:5,0.569)
--(axis cs:5,0.705)
--(axis cs:5,0.705)
--(axis cs:4,0.714)
--(axis cs:3,0.722)
--(axis cs:2,0.715)
--(axis cs:1,0.739)
--(axis cs:0,0.87)
--cycle;

\path [draw=color3, fill=color3, opacity=0.2]
(axis cs:0,0.884)
--(axis cs:0,0.868)
--(axis cs:1,0.818)
--(axis cs:2,0.761)
--(axis cs:3,0.744)
--(axis cs:4,0.746)
--(axis cs:5,0.682)
--(axis cs:5,0.73)
--(axis cs:5,0.73)
--(axis cs:4,0.766)
--(axis cs:3,0.778)
--(axis cs:2,0.809)
--(axis cs:1,0.832)
--(axis cs:0,0.884)
--cycle;

\path [draw=color4, fill=color4, opacity=0.2]
(axis cs:0,0.792)
--(axis cs:0,0.736)
--(axis cs:1,0.489)
--(axis cs:2,0.504)
--(axis cs:3,0.358)
--(axis cs:4,0.385)
--(axis cs:5,0.451)
--(axis cs:5,0.583)
--(axis cs:5,0.583)
--(axis cs:4,0.615)
--(axis cs:3,0.66)
--(axis cs:2,0.754)
--(axis cs:1,0.733)
--(axis cs:0,0.792)
--cycle;

\path [draw=color5, fill=color5, opacity=0.2]
(axis cs:0,0.712)
--(axis cs:0,0.652)
--(axis cs:1,0.582)
--(axis cs:2,0.654)
--(axis cs:3,0.524)
--(axis cs:4,0.402)
--(axis cs:5,0.448)
--(axis cs:5,0.754)
--(axis cs:5,0.754)
--(axis cs:4,0.718)
--(axis cs:3,0.72)
--(axis cs:2,0.71)
--(axis cs:1,0.702)
--(axis cs:0,0.712)
--cycle;

\addplot [semithick, color0]
table {%
0 0.895
1 0.636
2 0.587
3 0.579
4 0.579
5 0.561
};
\addlegendentry{Softmax}
\addplot [semithick, color1]
table {%
0 0.872
1 0.666
2 0.56
3 0.624
4 0.652
5 0.615
};
\addlegendentry{Ensemble}
\addplot [semithick, color2]
table {%
0 0.865
1 0.692
2 0.64
3 0.639
4 0.636
5 0.637
};
\addlegendentry{SNGP}
\addplot [semithick, color3]
table {%
0 0.876
1 0.825
2 0.785
3 0.761
4 0.756
5 0.706
};
\addlegendentry{MC Dropout}
\addplot [semithick, color4]
table {%
0 0.764
1 0.611
2 0.629
3 0.509
4 0.5
5 0.517
};
\addlegendentry{MIR}
\addplot [semithick, color5]
table {%
0 0.682
1 0.642
2 0.682
3 0.622
4 0.56
5 0.601
};
\addlegendentry{DDU}

\nextgroupplot[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=white!80!black
},
title={rAULC},
ymin=-0.1553, ymax=0.9293,
xmajorticks=false,
corrupted cityscapes plots,  
]
\path [draw=color0, fill=color0, opacity=0.2]
(axis cs:0,0.88)
--(axis cs:0,0.868)
--(axis cs:1,0.197)
--(axis cs:2,0.019)
--(axis cs:3,-0.019)
--(axis cs:4,0.019)
--(axis cs:5,0.025)
--(axis cs:5,0.211)
--(axis cs:5,0.211)
--(axis cs:4,0.303)
--(axis cs:3,0.313)
--(axis cs:2,0.415)
--(axis cs:1,0.487)
--(axis cs:0,0.88)
--cycle;

\path [draw=color1, fill=color1, opacity=0.2]
(axis cs:0,0.849)
--(axis cs:0,0.847)
--(axis cs:1,0.382)
--(axis cs:2,0.116)
--(axis cs:3,0.167)
--(axis cs:4,0.139)
--(axis cs:5,0.089)
--(axis cs:5,0.229)
--(axis cs:5,0.229)
--(axis cs:4,0.271)
--(axis cs:3,0.319)
--(axis cs:2,0.336)
--(axis cs:1,0.468)
--(axis cs:0,0.849)
--cycle;

\path [draw=color2, fill=color2, opacity=0.2]
(axis cs:0,0.841)
--(axis cs:0,0.827)
--(axis cs:1,0.363)
--(axis cs:2,0.186)
--(axis cs:3,0.108)
--(axis cs:4,0.102)
--(axis cs:5,0.116)
--(axis cs:5,0.196)
--(axis cs:5,0.196)
--(axis cs:4,0.296)
--(axis cs:3,0.318)
--(axis cs:2,0.414)
--(axis cs:1,0.559)
--(axis cs:0,0.841)
--cycle;

\path [draw=color3, fill=color3, opacity=0.2]
(axis cs:0,0.861)
--(axis cs:0,0.839)
--(axis cs:1,0.742)
--(axis cs:2,0.607)
--(axis cs:3,0.536)
--(axis cs:4,0.522)
--(axis cs:5,0.347)
--(axis cs:5,0.515)
--(axis cs:5,0.515)
--(axis cs:4,0.604)
--(axis cs:3,0.62)
--(axis cs:2,0.711)
--(axis cs:1,0.764)
--(axis cs:0,0.861)
--cycle;

\path [draw=color4, fill=color4, opacity=0.2]
(axis cs:0,0.672)
--(axis cs:0,0.55)
--(axis cs:1,0.208)
--(axis cs:2,0.146)
--(axis cs:3,-0.097)
--(axis cs:4,-0.106)
--(axis cs:5,-0.013)
--(axis cs:5,0.159)
--(axis cs:5,0.159)
--(axis cs:4,0.248)
--(axis cs:3,0.357)
--(axis cs:2,0.572)
--(axis cs:1,0.562)
--(axis cs:0,0.672)
--cycle;

\path [draw=color5, fill=color5, opacity=0.2]
(axis cs:0,0.517)
--(axis cs:0,0.393)
--(axis cs:1,0.215)
--(axis cs:2,0.214)
--(axis cs:3,0.074)
--(axis cs:4,-0.066)
--(axis cs:5,0.001)
--(axis cs:5,0.303)
--(axis cs:5,0.303)
--(axis cs:4,0.234)
--(axis cs:3,0.318)
--(axis cs:2,0.37)
--(axis cs:1,0.411)
--(axis cs:0,0.517)
--cycle;

\addplot [semithick, color0]
table {%
0 0.874
1 0.342
2 0.217
3 0.147
4 0.161
5 0.118
};
%\addlegendentry{softmax}
\addplot [semithick, color1]
table {%
0 0.848
1 0.425
2 0.226
3 0.243
4 0.205
5 0.159
};
%\addlegendentry{ensemble}
\addplot [semithick, color2]
table {%
0 0.834
1 0.461
2 0.3
3 0.213
4 0.199
5 0.156
};
%\addlegendentry{sngp}
\addplot [semithick, color3]
table {%
0 0.85
1 0.753
2 0.659
3 0.578
4 0.563
5 0.431
};
%\addlegendentry{dropout}
\addplot [semithick, color4]
table {%
0 0.611
1 0.385
2 0.359
3 0.13
4 0.071
5 0.073
};
%\addlegendentry{mir}
\addplot [semithick, color5]
table {%
0 0.455
1 0.313
2 0.292
3 0.196
4 0.084
5 0.152
};
%\addlegendentry{ddu}
\end{groupplot}

\end{tikzpicture}


==> figures/cityscapes_c_main/motion_blur.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color2}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color3}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}
\definecolor{color4}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color5}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=white!80!black
},
title={},
ymin=0.1458, ymax=0.5462,
xlabel={Severity},
corrupted cityscapes plots,
]
\path [draw=color0, fill=color0, opacity=0.2]
(axis cs:0,0.52)
--(axis cs:0,0.484)
--(axis cs:1,0.438)
--(axis cs:2,0.409)
--(axis cs:3,0.372)
--(axis cs:4,0.259)
--(axis cs:5,0.221)
--(axis cs:5,0.295)
--(axis cs:5,0.295)
--(axis cs:4,0.315)
--(axis cs:3,0.4)
--(axis cs:2,0.441)
--(axis cs:1,0.48)
--(axis cs:0,0.52)
--cycle;

\path [draw=color1, fill=color1, opacity=0.2]
(axis cs:0,0.528)
--(axis cs:0,0.522)
--(axis cs:1,0.464)
--(axis cs:2,0.421)
--(axis cs:3,0.383)
--(axis cs:4,0.323)
--(axis cs:5,0.284)
--(axis cs:5,0.334)
--(axis cs:5,0.334)
--(axis cs:4,0.349)
--(axis cs:3,0.399)
--(axis cs:2,0.429)
--(axis cs:1,0.486)
--(axis cs:0,0.528)
--cycle;

\path [draw=color2, fill=color2, opacity=0.2]
(axis cs:0,0.528)
--(axis cs:0,0.51)
--(axis cs:1,0.482)
--(axis cs:2,0.422)
--(axis cs:3,0.363)
--(axis cs:4,0.259)
--(axis cs:5,0.197)
--(axis cs:5,0.237)
--(axis cs:5,0.237)
--(axis cs:4,0.333)
--(axis cs:3,0.395)
--(axis cs:2,0.448)
--(axis cs:1,0.498)
--(axis cs:0,0.528)
--cycle;

\path [draw=color3, fill=color3, opacity=0.2]
(axis cs:0,0.514)
--(axis cs:0,0.498)
--(axis cs:1,0.486)
--(axis cs:2,0.471)
--(axis cs:3,0.455)
--(axis cs:4,0.428)
--(axis cs:5,0.402)
--(axis cs:5,0.432)
--(axis cs:5,0.432)
--(axis cs:4,0.444)
--(axis cs:3,0.475)
--(axis cs:2,0.495)
--(axis cs:1,0.506)
--(axis cs:0,0.514)
--cycle;

\path [draw=color4, fill=color4, opacity=0.2]
(axis cs:0,0.517)
--(axis cs:0,0.491)
--(axis cs:1,0.449)
--(axis cs:2,0.43)
--(axis cs:3,0.339)
--(axis cs:4,0.266)
--(axis cs:5,0.227)
--(axis cs:5,0.303)
--(axis cs:5,0.303)
--(axis cs:4,0.35)
--(axis cs:3,0.375)
--(axis cs:2,0.45)
--(axis cs:1,0.479)
--(axis cs:0,0.517)
--cycle;

\path [draw=color5, fill=color5, opacity=0.2]
(axis cs:0,0.519)
--(axis cs:0,0.491)
--(axis cs:1,0.437)
--(axis cs:2,0.365)
--(axis cs:3,0.28)
--(axis cs:4,0.194)
--(axis cs:5,0.164)
--(axis cs:5,0.232)
--(axis cs:5,0.232)
--(axis cs:4,0.254)
--(axis cs:3,0.334)
--(axis cs:2,0.405)
--(axis cs:1,0.463)
--(axis cs:0,0.519)
--cycle;

\addplot [semithick, color0]
table {%
0 0.502
1 0.459
2 0.425
3 0.386
4 0.287
5 0.258
};
%\addlegendentry{softmax}
\addplot [semithick, color1]
table {%
0 0.525
1 0.475
2 0.425
3 0.391
4 0.336
5 0.309
};
%\addlegendentry{ensemble}
\addplot [semithick, color2]
table {%
0 0.519
1 0.49
2 0.435
3 0.379
4 0.296
5 0.217
};
%\addlegendentry{sngp}
\addplot [semithick, color3]
table {%
0 0.506
1 0.496
2 0.483
3 0.465
4 0.436
5 0.417
};
%\addlegendentry{dropout}
\addplot [semithick, color4]
table {%
0 0.504
1 0.464
2 0.44
3 0.357
4 0.308
5 0.265
};
%\addlegendentry{mir}
\addplot [semithick, color5]
table {%
0 0.505
1 0.45
2 0.385
3 0.307
4 0.224
5 0.198
};
%\addlegendentry{ddu}

\nextgroupplot[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=white!80!black
},
title={},
ymin=0.6059, ymax=0.9161,
xlabel={Severity},
corrupted cityscapes plots,
]
\path [draw=color0, fill=color0, opacity=0.2]
(axis cs:0,0.899)
--(axis cs:0,0.891)
--(axis cs:1,0.89)
--(axis cs:2,0.886)
--(axis cs:3,0.871)
--(axis cs:4,0.828)
--(axis cs:5,0.814)
--(axis cs:5,0.854)
--(axis cs:5,0.854)
--(axis cs:4,0.862)
--(axis cs:3,0.881)
--(axis cs:2,0.896)
--(axis cs:1,0.902)
--(axis cs:0,0.899)
--cycle;

\path [draw=color1, fill=color1, opacity=0.2]
(axis cs:0,0.873)
--(axis cs:0,0.871)
--(axis cs:1,0.867)
--(axis cs:2,0.864)
--(axis cs:3,0.835)
--(axis cs:4,0.782)
--(axis cs:5,0.78)
--(axis cs:5,0.812)
--(axis cs:5,0.812)
--(axis cs:4,0.826)
--(axis cs:3,0.839)
--(axis cs:2,0.878)
--(axis cs:1,0.879)
--(axis cs:0,0.873)
--cycle;

\path [draw=color2, fill=color2, opacity=0.2]
(axis cs:0,0.87)
--(axis cs:0,0.86)
--(axis cs:1,0.856)
--(axis cs:2,0.861)
--(axis cs:3,0.849)
--(axis cs:4,0.84)
--(axis cs:5,0.818)
--(axis cs:5,0.856)
--(axis cs:5,0.856)
--(axis cs:4,0.88)
--(axis cs:3,0.871)
--(axis cs:2,0.883)
--(axis cs:1,0.874)
--(axis cs:0,0.87)
--cycle;

\path [draw=color3, fill=color3, opacity=0.2]
(axis cs:0,0.884)
--(axis cs:0,0.868)
--(axis cs:1,0.868)
--(axis cs:2,0.867)
--(axis cs:3,0.862)
--(axis cs:4,0.855)
--(axis cs:5,0.855)
--(axis cs:5,0.871)
--(axis cs:5,0.871)
--(axis cs:4,0.875)
--(axis cs:3,0.876)
--(axis cs:2,0.883)
--(axis cs:1,0.886)
--(axis cs:0,0.884)
--cycle;

\path [draw=color4, fill=color4, opacity=0.2]
(axis cs:0,0.792)
--(axis cs:0,0.736)
--(axis cs:1,0.746)
--(axis cs:2,0.732)
--(axis cs:3,0.698)
--(axis cs:4,0.664)
--(axis cs:5,0.636)
--(axis cs:5,0.734)
--(axis cs:5,0.734)
--(axis cs:4,0.752)
--(axis cs:3,0.776)
--(axis cs:2,0.762)
--(axis cs:1,0.788)
--(axis cs:0,0.792)
--cycle;

\path [draw=color5, fill=color5, opacity=0.2]
(axis cs:0,0.712)
--(axis cs:0,0.652)
--(axis cs:1,0.658)
--(axis cs:2,0.645)
--(axis cs:3,0.646)
--(axis cs:4,0.62)
--(axis cs:5,0.621)
--(axis cs:5,0.699)
--(axis cs:5,0.699)
--(axis cs:4,0.73)
--(axis cs:3,0.718)
--(axis cs:2,0.727)
--(axis cs:1,0.718)
--(axis cs:0,0.712)
--cycle;

\addplot [semithick, color0]
table {%
0 0.895
1 0.896
2 0.891
3 0.876
4 0.845
5 0.834
};
%\addlegendentry{softmax}
\addplot [semithick, color1]
table {%
0 0.872
1 0.873
2 0.871
3 0.837
4 0.804
5 0.796
};
%\addlegendentry{ensemble}
\addplot [semithick, color2]
table {%
0 0.865
1 0.865
2 0.872
3 0.86
4 0.86
5 0.837
};
%\addlegendentry{sngp}
\addplot [semithick, color3]
table {%
0 0.876
1 0.877
2 0.875
3 0.869
4 0.865
5 0.863
};
%\addlegendentry{dropout}
\addplot [semithick, color4]
table {%
0 0.764
1 0.767
2 0.747
3 0.737
4 0.708
5 0.685
};
%\addlegendentry{mir}
\addplot [semithick, color5]
table {%
0 0.682
1 0.688
2 0.686
3 0.682
4 0.675
5 0.66
};
%\addlegendentry{ddu}

\nextgroupplot[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.91,0.5)},
  anchor=east,
  draw=white!80!black
},
title={},
ymin=0.2709, ymax=0.9111,
xlabel={Severity},
corrupted cityscapes plots,
]
\path [draw=color0, fill=color0, opacity=0.2]
(axis cs:0,0.879)
--(axis cs:0,0.869)
--(axis cs:1,0.868)
--(axis cs:2,0.86)
--(axis cs:3,0.835)
--(axis cs:4,0.762)
--(axis cs:5,0.736)
--(axis cs:5,0.802)
--(axis cs:5,0.802)
--(axis cs:4,0.822)
--(axis cs:3,0.853)
--(axis cs:2,0.874)
--(axis cs:1,0.882)
--(axis cs:0,0.879)
--cycle;

\path [draw=color1, fill=color1, opacity=0.2]
(axis cs:0,0.851)
--(axis cs:0,0.847)
--(axis cs:1,0.839)
--(axis cs:2,0.833)
--(axis cs:3,0.791)
--(axis cs:4,0.711)
--(axis cs:5,0.699)
--(axis cs:5,0.753)
--(axis cs:5,0.753)
--(axis cs:4,0.777)
--(axis cs:3,0.801)
--(axis cs:2,0.853)
--(axis cs:1,0.855)
--(axis cs:0,0.851)
--cycle;

\path [draw=color2, fill=color2, opacity=0.2]
(axis cs:0,0.841)
--(axis cs:0,0.827)
--(axis cs:1,0.821)
--(axis cs:2,0.823)
--(axis cs:3,0.806)
--(axis cs:4,0.779)
--(axis cs:5,0.735)
--(axis cs:5,0.809)
--(axis cs:5,0.809)
--(axis cs:4,0.839)
--(axis cs:3,0.832)
--(axis cs:2,0.855)
--(axis cs:1,0.845)
--(axis cs:0,0.841)
--cycle;

\path [draw=color3, fill=color3, opacity=0.2]
(axis cs:0,0.862)
--(axis cs:0,0.84)
--(axis cs:1,0.841)
--(axis cs:2,0.839)
--(axis cs:3,0.825)
--(axis cs:4,0.819)
--(axis cs:5,0.811)
--(axis cs:5,0.839)
--(axis cs:5,0.839)
--(axis cs:4,0.845)
--(axis cs:3,0.849)
--(axis cs:2,0.861)
--(axis cs:1,0.865)
--(axis cs:0,0.862)
--cycle;

\path [draw=color4, fill=color4, opacity=0.2]
(axis cs:0,0.672)
--(axis cs:0,0.552)
--(axis cs:1,0.562)
--(axis cs:2,0.523)
--(axis cs:3,0.52)
--(axis cs:4,0.473)
--(axis cs:5,0.408)
--(axis cs:5,0.554)
--(axis cs:5,0.554)
--(axis cs:4,0.581)
--(axis cs:3,0.622)
--(axis cs:2,0.637)
--(axis cs:1,0.672)
--(axis cs:0,0.672)
--cycle;

\path [draw=color5, fill=color5, opacity=0.2]
(axis cs:0,0.515)
--(axis cs:0,0.393)
--(axis cs:1,0.399)
--(axis cs:2,0.405)
--(axis cs:3,0.423)
--(axis cs:4,0.3)
--(axis cs:5,0.348)
--(axis cs:5,0.502)
--(axis cs:5,0.502)
--(axis cs:4,0.534)
--(axis cs:3,0.519)
--(axis cs:2,0.541)
--(axis cs:1,0.535)
--(axis cs:0,0.515)
--cycle;

\addplot [semithick, color0]
table {%
0 0.874
1 0.875
2 0.867
3 0.844
4 0.792
5 0.769
};
%\addlegendentry{softmax}
\addplot [semithick, color1]
table {%
0 0.849
1 0.847
2 0.843
3 0.796
4 0.744
5 0.726
};
%\addlegendentry{ensemble}
\addplot [semithick, color2]
table {%
0 0.834
1 0.833
2 0.839
3 0.819
4 0.809
5 0.772
};
%\addlegendentry{sngp}
\addplot [semithick, color3]
table {%
0 0.851
1 0.853
2 0.85
3 0.837
4 0.832
5 0.825
};
%\addlegendentry{dropout}
\addplot [semithick, color4]
table {%
0 0.612
1 0.617
2 0.58
3 0.571
4 0.527
5 0.481
};
%\addlegendentry{mir}
\addplot [semithick, color5]
table {%
0 0.454
1 0.467
2 0.473
3 0.471
4 0.417
5 0.425
};
%\addlegendentry{ddu}
\end{groupplot}

\end{tikzpicture}


==> figures/image_classification/supplementary_regularization_strength/cifar10_regularization_strength.tex <==
\begin{figure}[t]
\centering
\setlength{\tabcolsep}{-7pt}
\resizebox{1.1\linewidth}{!}{
\begin{tabular}{cccc}
% \vspace{-4mm}
% \hspace{-3mm}
\input{figures/image_classification/regularization_strength/dropout_cifar10_AULC_additive_gaussian_vs_ACC} & \hspace{1mm}
\input{figures/image_classification/regularization_strength/dropout_cifar10_AULC_jpeg_quality_vs_ACC} & 
\input{figures/image_classification/regularization_strength/dropout_cifar10_stl10_AUROC_vs_ACC}  & \hspace{-6mm}
\input{figures/image_classification/regularization_strength/dropout_cifar10_svhn_cropped_AUROC_vs_ACC} 
\\ \vspace{-1mm}
\input{figures/image_classification/regularization_strength/duq_cifar10_AULC_additive_gaussian_vs_ACC} &  \hspace{1mm}
\input{figures/image_classification/regularization_strength/duq_cifar10_AULC_jpeg_quality_vs_ACC} & \hspace{0mm}
\input{figures/image_classification/regularization_strength/duq_cifar10_stl10_AUROC_vs_ACC}  & \hspace{1mm}
\input{figures/image_classification/regularization_strength/duq_cifar10_svhn_cropped_AUROC_vs_ACC}
\\ \vspace{-1mm}
\input{figures/image_classification/regularization_strength/sngp_cifar10_AULC_additive_gaussian_vs_ACC} &  \hspace{1mm}
\input{figures/image_classification/regularization_strength/sngp_cifar10_AULC_jpeg_quality_vs_ACC} & 
\input{figures/image_classification/regularization_strength/sngp_cifar10_stl10_AUROC_vs_ACC}  & \hspace{-6mm}
\input{figures/image_classification/regularization_strength/sngp_cifar10_svhn_cropped_AUROC_vs_ACC}
\\ \vspace{-1mm}
\input{figures/image_classification/regularization_strength/mir_cifar10_AULC_additive_gaussian_vs_ACC} & \hspace{1mm}
\input{figures/image_classification/regularization_strength/mir_cifar10_AULC_jpeg_quality_vs_ACC} & \hspace{1mm}
\input{figures/image_classification/regularization_strength/mir_cifar10_stl10_AUROC_vs_ACC}  & \hspace{-6mm}
\input{figures/image_classification/regularization_strength/mir_cifar10_svhn_cropped_AUROC_vs_ACC}  
\\ \vspace{-1mm}
\end{tabular}
}
\vspace{-0.5em}
\caption{Trained on CIFAR10. Vertical axis: Test accuracy. Horizontal axis: \ac{raulc} against additive gaussian noise (1st column) and additive jpeg quality corruption (2nd column), \ac{auroc} against STL10 (3rd column) and SVHN (4th column) for Dropout (1st row), DUQ (2nd row), SNGP (3rd row) and MIR (4th row) using different regularization strength. For SNGP a larger hyperparameter corresponds to less regularization. For Dropout we observe a correlation between regularization strength and performance.}\label{fig:suppl_cifar_sensitivity_to_regularization_strength}
\vspace{-1em}
\end{figure}

==> figures/image_classification/supplementary_regularization_strength/svhn_regularization_strength.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{-7pt}
\resizebox{1.1\linewidth}{!}{
\begin{tabular}{cccc}
% \vspace{-4mm}
\input{figures/image_classification/regularization_strength/dropout_svhn_AULC_additive_gaussian_vs_ACC} &
\input{figures/image_classification/regularization_strength/dropout_svhn_AULC_jpeg_quality_vs_ACC} &
\input{figures/image_classification/regularization_strength/dropout_svhn_cifar10_AUROC_vs_ACC}  & \hspace{-4mm}
\input{figures/image_classification/regularization_strength/dropout_svhn_stl10_AUROC_vs_ACC} 
\\ \vspace{-1mm}
\hspace{-3mm}\input{figures/image_classification/regularization_strength/duq_svhn_AULC_additive_gaussian_vs_ACC} & 
\input{figures/image_classification/regularization_strength/duq_svhn_AULC_jpeg_quality_vs_ACC} & \hspace{1mm}
\input{figures/image_classification/regularization_strength/duq_svhn_cifar10_AUROC_vs_ACC}  & \hspace{-1mm}
\input{figures/image_classification/regularization_strength/duq_svhn_stl10_AUROC_vs_ACC}
\\ \vspace{-1mm}
\input{figures/image_classification/regularization_strength/sngp_svhn_AULC_additive_gaussian_vs_ACC} & 
\input{figures/image_classification/regularization_strength/sngp_svhn_AULC_jpeg_quality_vs_ACC} & 
\input{figures/image_classification/regularization_strength/sngp_svhn_cifar10_AUROC_vs_ACC}  & \hspace{-4mm}
\input{figures/image_classification/regularization_strength/sngp_svhn_stl10_AUROC_vs_ACC}
\\ \vspace{-1mm}
\input{figures/image_classification/regularization_strength/mir_svhn_AULC_additive_gaussian_vs_ACC} & 
\input{figures/image_classification/regularization_strength/mir_svhn_AULC_jpeg_quality_vs_ACC} &
\input{figures/image_classification/regularization_strength/mir_svhn_cifar10_AUROC_vs_ACC}  & \hspace{-4mm}
\input{figures/image_classification/regularization_strength/mir_svhn_stl10_AUROC_vs_ACC}  
\\ \vspace{-1mm}
\end{tabular}
}
\vspace{-0.5em}
\caption{Trained on SVHN. Vertical axis: Test accuracy. Horizontal axis: \ac{raulc} against additive gaussian noise (1st column) and additive jpeg quality corruption (2nd column), \ac{auroc} against CIFAR10 (3rd column) and STL10 (4th column) for Dropout (1st row), DUQ (2nd row), SNGP (3rd row) and MIR (4th row) using different regularization strength. For SNGP a larger hyperparameter corresponds to less regularization. For Dropout we observe a correlation between regularization strength and performance.}\label{fig:suppl_svhn_sensitivity_to_regularization_strength}
\vspace{-1em}
\end{table}

==> figures/supplementary_segmentation_uncertainty/minimal_shift_uncertainty_old.tex <==
\begin{figure}[t]
\centering
\setlength{\tabcolsep}{3pt}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
% \renewcommand{\arraystretch}{3}
% \resizebox{1.1\linewidth}{!}{
\begin{tabular}{cccccc}
% \vspace{-4mm}
% \hspace{-3mm}
 & Input & GT & Prediction & Error & Uncertainty \\
\hline\addlinespace[2pt]
\multirow{2}{*}{\rotatebox[origin=c]{90}{Softmax}} &
% \\[\dimexpr-\normalbaselineskip+2pt] &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/softmax_time_of_the_day/perturbation_85/0_img.png} & 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/softmax_time_of_the_day/perturbation_85/0_targ.png} & 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/softmax_time_of_the_day/perturbation_85/0_pred.png} &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/softmax_time_of_the_day/perturbation_85/0_err.png} &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/softmax_time_of_the_day/perturbation_85/0_unc.png} 
\\ 
& 
% \\[\dimexpr-\normalbaselineskip+2pt] &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/softmax_time_of_the_day/perturbation_85/1_img.png} & 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/softmax_time_of_the_day/perturbation_85/1_targ.png} & 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/softmax_time_of_the_day/perturbation_85/1_pred.png} &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/softmax_time_of_the_day/perturbation_85/1_err.png} &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/softmax_time_of_the_day/perturbation_85/1_unc.png} 
\\
\hline\addlinespace[2pt]
\multirow{2}{*}{\rotatebox[origin=c]{90}{Dropout}} &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/dropout_time_of_the_day/perturbation_85/0_img.png} & 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/dropout_time_of_the_day/perturbation_85/0_targ.png} & 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/dropout_time_of_the_day/perturbation_85/0_pred.png} &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/dropout_time_of_the_day/perturbation_85/0_err.png} &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/dropout_time_of_the_day/perturbation_85/0_unc.png} 
\\
& 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/dropout_time_of_the_day/perturbation_85/1_img.png} & 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/dropout_time_of_the_day/perturbation_85/1_targ.png} & 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/dropout_time_of_the_day/perturbation_85/1_pred.png} &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/dropout_time_of_the_day/perturbation_85/1_err.png} &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/dropout_time_of_the_day/perturbation_85/1_unc.png} 
\\
\hline\addlinespace[2pt]
\multirow{2}{*}{\rotatebox[origin=c]{90}{SNGP}} &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/sngp_time_of_the_day/perturbation_85/0_img.png} & 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/sngp_time_of_the_day/perturbation_85/0_targ.png} & 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/sngp_time_of_the_day/perturbation_85/0_pred.png} &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/sngp_time_of_the_day/perturbation_85/0_err.png} &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/sngp_time_of_the_day/perturbation_85/0_unc.png} 
\\
& 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/sngp_time_of_the_day/perturbation_85/1_img.png} & 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/sngp_time_of_the_day/perturbation_85/1_targ.png} & 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/sngp_time_of_the_day/perturbation_85/1_pred.png} &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/sngp_time_of_the_day/perturbation_85/1_err.png} &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/sngp_time_of_the_day/perturbation_85/1_unc.png} 
\\
\hline\addlinespace[2pt]
\multirow{2}{*}{\rotatebox[origin=c]{90}{MIR}} & 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/mir_time_of_the_day/perturbation_85/0_img.png} & 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/mir_time_of_the_day/perturbation_85/0_targ.png} & 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/mir_time_of_the_day/perturbation_85/0_pred.png} &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/mir_time_of_the_day/perturbation_85/0_err.png} &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/mir_time_of_the_day/perturbation_85/0_unc.png} 
\\
& 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/mir_time_of_the_day/perturbation_85/1_img.png} & 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/mir_time_of_the_day/perturbation_85/1_targ.png} & 
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/mir_time_of_the_day/perturbation_85/1_pred.png} &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/mir_time_of_the_day/perturbation_85/1_err.png} &
\includegraphics[width=2.5cm,trim={2.1cm 2.15cm 1.65cm 2.5cm},clip]{figures/supplementary_segmentation_uncertainty/images/mir_time_of_the_day/perturbation_85/1_unc.png} 
\\
\end{tabular}
% }
\vspace{-0.5em}
\caption{Minimal distribution shift.}\label{fig:suppl_segmentation_85
}
\vspace{-1em}
\end{figure}

==> sections_old/0_abstract.tex <==
\iffalse
\begin{abstract}
  Recently a set of novel approaches to epistemic uncertainty estimation in deep neural networks, which we term deterministic uncertainty (DU), has emerged as a valid alternative to Bayesian Neural Networks (BNNs). On the premise of informative representations, these achieve strong performance on detecting out-of-distribution (OOD) data while adding negligible computational costs at inference time. However, thus far it remains unclear whether DU is well calibrated under continuous distribution shifts and scales to real-world applications, both of which are prerequisites for practical deployment. To this end, we provide a taxonomy of DU and benchmark various approaches on image classification regarding OOD detection and calibration under continuous distribution shifts. In addition, we demonstrate that DU scales to realistic vision tasks while providing trustworthy epistemic uncertainty. Therefore, we extend the most promising approaches to semantic segmentation and benchmark them on realistic continuous distributional shifts using simulated data.
\end{abstract}
\fi

% New version
% \begin{abstract}
%   A set of novel approaches for estimating epistemic uncertainty in deep neural networks with a single forward pass has recently emerged as a valid alternative to Bayesian Neural Networks. On the premise of informative representations, these deterministic uncertainty methods (DUMs) achieve strong performance on detecting out-of-distribution (OOD) data while adding negligible computational costs at inference time. However, so far it remains unclear whether DUMs are well calibrated under continuous distributional shifts and can seamlessly scale to real-world applications - both prerequisites for their practical deployment. To this end, we firstly provide a taxonomy of DUMs and evaluate their calibration under continuous distributional shifts and the performance on OOD detection for image classification tasks. Then, we extend the most promising approaches to semantic segmentation and demonstrate that DUMs scale to realistic vision tasks, while providing trustworthy epistemic uncertainty under realistic continuous distributional shifts.
% \end{abstract}

\begin{abstract}
  A set of novel approaches for estimating epistemic uncertainty in deep neural networks with a single forward pass has recently emerged as a valid alternative to Bayesian Neural Networks. On the premise of informative representations, these deterministic uncertainty methods (DUMs) achieve strong performance on detecting out-of-distribution (OOD) data while adding negligible computational costs at inference time. However, it remains unclear whether DUMs are well calibrated and can seamlessly scale to real-world applications - both prerequisites for their practical deployment.
  %
  To this end, we first provide a taxonomy of DUMs, evaluate their calibration under continuous distributional shifts and their performance on OOD detection for image classification tasks. 
  %
  Then, we extend them to semantic segmentation. 
  %
  We find that, while DUMs scale to realistic vision tasks and perform well on OOD detection, the practicality of current methods is undermined by suboptimal calibration under realistic distributional shifts.
\end{abstract}

==> sections_old/1_introduction.tex <==
%
Despite the dramatic enhancement of predictive performance by \ac{dl}, its adoption remains limited due to unpredictable failure on \ac{ood} samples~\cite{blanchard2011generalizing,muandet2013domain} and adversarial attacks~\cite{szegedy2013intriguing}.
%
Uncertainty estimation techniques aim at bridging this gap by providing accurate confidence levels on a model's output, allowing for a safe deployment of \acp{nn} in life-critical tasks, \eg{} autonomous driving or medical applications.
% , and can also foster effective policies for exploration in reinforcement learning.

While \acp{bnn} represent the predominant holistic solution for quantifying uncertainty~\cite{hinton1993keeping,neal2012bayesian}, exactly modelling their full posterior is often intractable, and scalable versions usually require expensive variational approximations~\cite{kingma2015variational,gal2016dropout,zhang2018noisy,postels2019sampling,loquercio2020general}.
%
Moreover, it has recently been shown that true Bayes posterior usually leads to poor uncertainty~\cite{wenzel2020good}.
%
Thus, efficient approaches to uncertainty estimation largely remain an open problem, limiting the adoption in real-time applications with strict memory, time and safety requirements.

%
Recently, a promising line of work emerged to estimate epistemic uncertainty in deterministic \acp{nn} with a single forward pass.
%
By regularizing the hidden representations of a model, these methods represent an efficient and scalable solution to epistemic uncertainty estimation and to the related \ac{ood} detection problem.
%
Compared to traditional uncertainty estimation techniques, \acp{dum} quantify epistemic uncertainty by measuring distances~\cite{mandelbaum2017distance,van2020uncertainty} or estimating the distribution of latent representations~\cite{alemi2018uncertainty, liu2020simple, wu2020simple, charpentier2020posterior, van2021improving, mukhoti2021deterministic, postels2020hidden, charpentier2021natural}.
%
While \ac{ood} detection arguably enables a safe deployment of \ac{dl} also in previously unseen scenarios, we argue that evaluating the calibration - \ie{} how well uncertainty correlates with model performance - of such methods in proximity of the training distribution and under continuous distributional shift is equally important.
%
Nonetheless, we observe that previous work on \acp{dum} falls short of investigating calibration, and solely focus on \ac{ood} detection~\cite{mandelbaum2017distance,van2020uncertainty,wu2020simple,van2021improving, mukhoti2021deterministic}. 
%
Further, such techniques have only been evaluated on toy datasets for binary classification or small-scale image classification tasks \cite{van2020uncertainty, mukhoti2021deterministic}.
%
Despite claiming to solve practical issues of traditional uncertainty estimation approaches, the practicality of \acp{dum} remains to be assessed on more challenging tasks.

This work aims to give an answer to some of the most crucial questions on the use of \acp{dum} and address shortcomings and scalability issues. 
%
In particular:
%
(i) to the best of our knowledge, we are the first to analyze the calibration of \acp{dum} under continuous distributional shifts;
%
(ii) we evaluate the quality of \acp{dum} for \ac{ood} detection and their sensitivity to regularization strength;
%
% (iii) we show how maximising the informativeness of hidden representations yields superior deterministic uncertainty compared to enforcing distance preserving features;
%
(iii) we scale promising deterministic uncertainty methods to dense prediction tasks, \eg{} semantic segmentation, and evaluate them on sequences collected in the CARLA simulator~\cite{Dosovitskiy17} under realistic continuous distributional shift;
%
% (iv) we show how current \acp{dum} are better calibrated than softmax models, but are still suboptimal compared to probabilistic methods such as Monte-Carlo dropout~\cite{gal2016dropout}.
(iv) we show how the practicality of current \acp{dum} is undermined by their poor calibration under realistic distributional shifts.
% compared to Monte-Carlo dropout~\cite{gal2016dropout}.

\vspace{-3mm}


==> sections_old/2_related_work.tex <==
\textbf{Sources of Uncertainty.} 
Uncertainty in a model's predictions can arise from two different sources~\cite{der2009aleatory, kendall2017uncertainties}.
%
While \textit{aleatoric} uncertainty encompasses the noise inherent in the data and is consequently irreducible~\cite{der2009aleatory}, \textit{epistemic} uncertainty quantifies the uncertainty associated with choosing the model parameters based on limited information, and vanishes - in principle - in the limit of infinite data.
%
%A well-calibrated uncertainty estimate is expected to provide low values for correct predictions, and increasingly higher uncertainty values as the model performance degrades.
%
This work distinguishes two properties of epistemic uncertainty - its performance on detecting \ac{ood} samples and its calibration (\ie its correlation with model performance under distributional shifts). While the latter has been explored in the case of probabilistic approaches to uncertainty estimation \cite{snoek2019can}, to the best of our knowledge, we are the first to investigate the behaviour of \acp{dum} in this scenario. Notably, \cite{gustafsson2020evaluating} evaluates prominent scalable epistemic uncertainty estimates on semantic segmentation. However, they investigate calibration only on in-distribution data. 
% Note that although \cite{liu2020simple} evaluates the calibration of their approach, they do so exclusively on in-distribution data. 

\noindent\textbf{\acp{bnn}}~\cite{neal2011mcmc,neal2012bayesian} represent a principled way of measuring uncertainty. 
%
However, the intractability of their posterior distribution requires approximate inference methods, such as Markov Chain Monte-Carlo~\cite{neal2011mcmc} or \ac{vi}~\cite{hinton1993keeping}. While these methods traditionally struggle with large datasets and architectures, a variety of scalable approaches - often based on \ac{vi} - has recently emerged. 


%~\cite{hinton1993keeping,kingma2015variational, gal2016dropout,zhang2018noisy,teye2018bayesian}.
%
%These methods either require expensive Monte-Carlo sampling or are unable to scale to large datasets and architectures.
%

\noindent\textbf{Deep Ensembles}, which typically consist of identical models trained from different initializations,
%The current state-of-the art in uncertainty estimation in deep learning is represented by ensemble models.
%
have been introduced to the deep learning community by Lakshminarayanan \etal~\cite{lakshminarayanan2017simple} and extended by~\cite{wen2020batchensemble,dusenberry2020efficient}. 
% Moreover, deep ensembles are related to \acp{bnn} when viewed through the lense of Bayesian model averaging~\cite{wilson2020bayesian}. 
While deep ensembles are widely regarded as a strong baseline for estimating epistemic uncertainty, they come with a high computational costs as well as their memory footprint.

\textbf{Efficient Approaches.}
%To reduce the computational overload and memory consumption of ensemble models and BNNs, several approaches to estimate uncertainty using just a single model have emerged.
%
%Some approaches exploit \textit{multiple forward passes} through a single model to simulate an ensemble of networks.
%
Recently, a variety of approaches based on stochastic regularization have been developed~\cite{kingma2015variational,gal2016dropout,zhang2018noisy,teye2018bayesian}.
By keeping stochasticity switched on at inference time, they estimate uncertainty using multiple forward passes. %The most prominent example is Monte-Carlo dropout~\cite{gal2016dropout}. Originally proposed as a bayesian approximation to represent model uncertainty, it allows to derive epistemic uncertainty from multiple forward passes through a single model by randomly dropping different neurons at every forward pass. 
%
Moreover, efficient ensemble methods were proposed producing predictions using a single model~\cite{rupprecht2017learning, dusenberry2020efficient, wen2020batchensemble}. 
%
Despite these methods show promising results on large-scale tasks while being parameter-efficient, they still need multiple forward passes through the model, which can render them impractical given a limited computational budget.
%
To enable uncertainty modelling in real-time and resource-demanding tasks, recent work has focused on providing uncertainty estimates with a \textit{single forward pass}.
%
% it is indeed essential to provide confidence measures at a high pace, and performing multiple forward passes can be prohibitive when memory and processing requirements are strict.  
%
%Some methods propose to mitigate overconfidence of softmax networks and provide high-quality epistemic uncertainty by replacing the loss function~\cite{hein2019relu, malinin2018predictive, sensoy2018evidential} or the output layer~\cite{bendale2016towards,tagasovska2018single,calandra2016manifold}. 
%
For instance, one line of work proposes a principled approach for variance propagation in \acp{nn}~\cite{postels2019sampling, haussmann2020sampling, loquercio2020general}. 
% or by computing a closed-form posterior for the output layer~\cite{kristiadi2020being,riquelme2018deep,snoek2015scalable}.

Recently, a new family of methods - \acp{dum} - showed promising results in uncertainty estimation for \ac{ood} detection.
%
By leveraging distances and densities in the feature space of a \ac{nn}, these methods provide confidence estimates while adding negligible computational cost.
%
Since they are united in their deterministic treatment of the weights, we term them Deterministic Uncertainty Methods (DUMs).
%
The next section provides a taxonomy of \acp{dum}, summarizing these recently emerging approaches to quantifying epistemic uncertainty.


==> sections_old/3_taxonomy.tex <==
% mandelbaum2017distance --> DCS (distance-based confidence score)
% alemi2018uncertainty --> VIB
% van2020uncertainty --> DUQ
% liu2020simple --> SNGP
% wu2020simple --> DUM
% van2021improving --> DUE
% mukhoti2021deterministic --> DDU
% postels2020hidden --> MIR
% nalisnick2019hybrid, ardizzone2020training --> invertible models
% TAXONOMY
% How to enforce Bi-Lipschitz regularization
% --> It is possible to reduce feature collapse by enforcing two constraints on the model: sensitivity and smoothness.
% Sensitivity implies that when the input changes the feature representation also changes: this means the model cannot simply collapse feature representations arbitrarily. 
%Smoothness means small changes in the input cannot cause massive shifts in the output. This appears to help optimization, and ensures the feature space accords with the implicit assumptions that for example RBF kernels make about the data.
%
%
% \input{tables/taxonomy}
%
% \input{tables/taxonomy_v1}
% %
% \input{tables/taxonomy_v2}
% %
% \input{tables/taxonomy_v3}
%
\input{tables/taxonomy_v4}
%
This section proposes a taxonomy of existing \acp{dum}.
%
To quantify epistemic uncertainty deterministically, the distribution of the hidden representations of a neural network needs to represent the input distribution.
%
However, discriminative models suffer from the fundamental problem of feature collapse. 
%
Thus, we firstly categorize \acp{dum} according to the regularization method used to counteract feature collapse (\autoref{ssec:taxonomy_strategy}).
%
Moreover, we cluster \acp{dum} according to the method used for uncertainty estimation (\autoref{ssec:taxonomy_density_models}).
%Finally, in \autoref{ssec:taxonomy_density_models} we detail how each method estimates uncertainty from the so-trained neural network.
%
%To facilitate the reader, we synthesize the proposed taxonomy in \autoref{table:taxonomy}.
\autoref{table:taxonomy} shows an overview of the resulting taxonomy.

%%%%%
\textbf{Feature Collapse.} \label{ssec:feature_collapse}
%
%Deterministic uncertainty methods typically rely on density estimation in the hidden space of a feature extractor to capture epistemic uncertainty.
%
%However, applying density models directly to the feature space does not work out of the box~\cite{mandelbaum2017distance}. 
%
Discriminative models can learn to discard large part of their input information, as exploiting spurious correlations may lead to better performance on the training data distribution~\cite{peters2017elements, segu2020batch}. 
%
The invariant representations learned by discriminative models extend to \ac{ood} data, resulting in a collapse of \ac{ood} embeddings to in-distribution features in the hidden space.
%
This problem is known as \textit{feature collapse}~\cite{van2020uncertainty}, and it makes \ac{ood} detection based on high-level representations impossible.
%
%Ideally, representations of \ac{ood} samples must be separable from in-distribution ones.
%
% 
% While this has proven to be effective on several toy datasets, it is unclear whether it can actually scale to more complicated tasks, \eg{} semantic segmentation.
%

\subsection{Regularization of Hidden Representations} \label{ssec:taxonomy_strategy}
We group \acp{dum} according to how feature collapse is tackled, enabling \ac{ood} detection based on latent representations.
%
In particular, we identify two main paradigms - distance awareness and informative representations - which we discuss in \autoref{sssec:distance_awareness} and \autoref{sssec:informative_representations}.

\subsubsection{Distance Awareness} \label{sssec:distance_awareness}

The fundamental idea of distance-aware hidden representations is to avoid feature collapse by enforcing distances between latent representations to mirror distances in the input space. 
%
This can be achieved by constraining the Lipschitz constant, as it enforces a lower and an upper bound to expansion and contraction performed by an underlying neural network. 
%
A lower bound is associated with \textit{sensitivity}, since it enforces that different inputs are mapped to distinct latent representations and, thus, provides a solution to feature collapse. 
%
Moreover, an upper bound enforces \textit{smoothness} of the hidden representations, \ie{} small changes in the input do not result in large changes in the latent space.
% More formally, typically a lower and upper bound is imposed over the resulting activation of a feature extractor $f_\theta$ with parameters $\theta$: $c_1||x_1=x_2||_I \leq ||f_\theta(x_1)-f_\theta(x_2)||_F \leq c_2||x_1=x_2||_I$, where this must hold for any pair of inputs $x_1$ and $x_2$.
% 
More formally, given any pair of inputs $x_1$ and $x_2$ the following lower and upper bounds must hold for the resulting activation of a feature extractor $f_\theta$ with parameters $\theta$: $c_1||x_1-x_2||_I \leq ||f_\theta(x_1)-f_\theta(x_2)||_F \leq c_2||x_1-x_2||_I$.
%
$c_1$ and $c_2$ denote respectively the lower and upper bound for the Lipschitz constant, and $||\cdot||_I$ and $||\cdot||_F$ are the chosen metrics in the input and feature space respectively.
%
%
% Mandelbaum \etal~\cite{mandelbaum2017distance} first attempted to enforce sensitive embeddings by proposing two alternative solutions - \ie{} adversarial examples augmentation and supervised distance-based contrastive learning - to increase the distance between pairs of training points with different labels.
%
While there exist other approaches, \eg{}~\cite{obukhov2021spectral}, recent proposals have primarily adopted two methods to impose the bi-Lipschitz constraint. 
%%%%%%%%%%%%%%%%%%

\textbf{Gradient Penalty.} 
%
First introduced to regularize the Lipschitz constant in GAN training~\cite{gulrajani2017improved}, a two-sided gradient penalty is used as an additional loss term to enforce detectability in the feature space of changes in the input by DUQ~\cite{van2020uncertainty}.
%
The gradient penalty is formulated as an additional loss term that regularises the Frobenius norm $||J||_F$ of the Jacobian $J$ of a \ac{nn} to enforce a bi-Lipschitz
constraint. Therefore, the training loss of a \ac{nn} is typically enhanced with the absolute difference between $||J||_F$ and some chosen positive constant (see supplement or \cite{van2020uncertainty} for more details).
% %
% Following this intuition, DUQ~\cite{van2020uncertainty} enforces detectability of changes in the input using the two-sided gradient penalty.

\textbf{Spectral Normalization.} The two-sided gradient penalty described above requires backpropagating through the Jacobian of a \ac{nn} and is, thus, computationally demanding. A more efficient technique is \ac{sn}~\cite{miyato2018spectral}. For each layer, \ac{sn} normalizes the weights $W$ of each layer using their spectral norm $sn(W)$ to constrain the bi-Lipschitz constant. Thus, weight matrices are normalized according to: $W_{sn}=\frac{W}{c\cdot sn(W)}$.
%
Note, that this soft constraint becomes hard for $c=1$. We refer to the supplement or \cite{liu2020simple} for further details.
%
Various \acp{dum} - SNGP~\cite{liu2020simple}, DUE~\cite{van2021improving} and DDU~\cite{mukhoti2021deterministic} - rely on \ac{sn} of the weight matrices to enforce distance-awareness of hidden representations.
%
%%%%%%%%%%%%%%%%%%%%%%%%%

%
% For a detailed description of gradient penalty and spectral normalization, please refer to the Appendix.
%
Note that the Lipschitz constraint is defined with respect to a predefined distance measure, which can be difficult to choose for many high-dimensional data distributions of practical interest.
%
A popular choice, also adopted by~\cite{van2020uncertainty,liu2020simple,van2021improving}, is the $L_2$ distance.
% which has been shown not to be particularly meaningful for image-based tasks~\cite{gouk2021regularisation}.
%
Moreover, principled approaches to provide exact singular values in convolutional layers~\cite{sedghi2018singular} result in prohibitive computational complexity; the spectral normalization approximations typically adopted by the methods previously described have been found to be sub-optimal~\etal~\cite{singla2019bounding}, and its interaction with losses, architecture and optimization is yet to be fully understood~\cite{rosca2020case}.
%
Consequently, Lipschitz regularization with respect to a potentially meaningless distance measure may result in overly sensitive models.
%
\autoref{ssec:classification_results} analyses the impact of regularization strength on \ac{ood} detection.

%
\subsubsection{Informative Representations} \label{sssec:informative_representations}
%
While methods enforcing distance-awareness achieve remarkable performance in OOD detection, they do not explicitly preserve sample-specific information.
%but only enforce distance awareness according to a predefined distance metric in the input space. 
%
Consequently, depending on the underlying distance metric they may discard useful information about the input or act overly sensitive.
%
An alternative line of work proposes to avoid feature collapse by learning informative representations~\cite{alemi2018uncertainty,wu2020simple,postels2020hidden,nalisnick2019hybrid,ardizzone2018analyzing,ardizzone2020training}, thus forcing discriminative models to preserve information beyond what required by its target task in its hidden representations independent of the choice of an underlying distance metric.
%
Notably, while representations that are aware of distances in the input space are arguably also informative, both categories remain fundamentally different in their approach to feature collapse.
%
While distance-awareness is based on the choice of a specific distance metric tying together input and latent space, informative representations incentivize the network to store more information about the input using an auxiliary task \cite{postels2020hidden, wu2020simple} or forbid information loss by construction \cite{ardizzone2018analyzing,nalisnick2019hybrid,ardizzone2020training}.
%enforce a constraint on the distribution of hidden representations.
%
We identify three distinct families of approaches to enforce informative representations.

%To this end, Alemi \etal~\cite{alemi2018uncertainty} propose to maximize in variational autoencoders the mutual information between the desired output and its representation to preserve each class from collapsing onto another. 
%
%Optimal representation must also reduce the mutual information between an input and its representation to contain uninformative variability.
%
\textbf{Contrastive learning}~\cite{oord2018representation,wu2020simple} has emerged as an approach for learning representations that are both informative and discriminative.
%
This is utilized by Wu \etal~\cite{wu2020simple}, who build on top of SimCLR~\cite{chen2020simple} to regularize hidden representations for a discriminative task by using an auxiliary contrastive loss to force representations to further discriminate between individual instances. 
% Subsequently, they estimate the distribution of hidden representations and use the log-likelihood of as an uncertianty proxy.

\textbf{Reconstruction regularization}~\cite{postels2020hidden} instead forces the intermediate activations to embody a complete representation of the input space. 
%
This is achieved by adding a decoder branch fed with the activations of a given layer to reconstruct the input.
%
% Consequently, the network's activations are not susceptible to feature collapse, since sample- and domain-specific features are retained in the hidden representations.
%
Since this method aims at producing Maximally Informative Representations, we term it MIR.
% 
% Compared to other approaches, MIR is in principle extendable to any architecture and avoids the strict constraints imposed by spectral normalization or gradient penalty.
%

\textbf{\acp{inn}}~\cite{jacobsen2018revnet,ardizzone2018analyzing,nalisnick2019hybrid,ardizzone2020training}, built via a cascade of homeomorphic layers, cannot discard information except at the final classification stage.
%
Consequently, the mutual information between input and hidden representation is retained by construction.
%
Interestingly, Behrmann \etal~\cite{behrmann2018invertible} showed that a ResNet is invertible if its Lipschitz constant is lower than $1$, meaning that invertible ResNets both possess highly-informative representations and satisfy distance-awareness. However, note that this is not a necessary condition for invertibility, and thus information preservation, in general.
%
% This property makes them an ideal candidate for \ac{ood} detection.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Uncertainty Estimation} \label{ssec:taxonomy_density_models}
We now describe the different approaches to quantifying uncertainty based on such regularized representations. 
%
We distinguish two directions - generative and discriminative approaches. 
%
While generative approaches use the likelihood produced by an explicit generative model of the distribution of hidden representations as a proxy for uncertainty, discriminative methods directly use the predictions based on regularized representations to quantify uncertainty.
%

\textbf{Generative approaches} estimate the distribution of hidden representations post-training and use the likelihood as uncertainty metric to detect \ac{ood} samples.
%
Wu \etal~\cite{wu2020simple} propose a Deep Contrastive Uncertainty (DCU) method to train an additional deep network from the representation space to a distribution space, where the variance of the distribution is used as a confidence measure.
%
MIR~\cite{postels2020hidden} and DDU~\cite{mukhoti2021deterministic} fit a class-conditional GMM to their regularized hidden representations and use the log-likelihood as an epistemic uncertainty proxy.
%
A special instance of the generative approaches are \acp{inn} as they directly estimate the training data distribution. This allows using the likelihood of the input data as a proxy of uncertainty. While this idea is appealing, it can lead to training difficulties, imposes strong constraints on the underlying feature extractor and in some instances even remains susceptible to \ac{ood} data~\cite{nalisnick2018deep}.

\textbf{Discriminative approaches} use the predictions based on regularized representations to directly assess confidence.
%
Mandelbaum \etal~\cite{mandelbaum2017distance} propose to use a Distance-based Confidence Score (DCS) to estimate local density at a point as the Euclidean distance in the embedded space between the point and its k nearest neighbors in the training set.
%
Similarly, DUQ~\cite{van2020uncertainty} builds on Radial Basis Function (RBF) networks~\cite{lecun1998gradient} and propose a novel centroid updating scheme. 
%
Uncertainty is estimated as the distance between the model output and the closest centroid.
%
DUMs adopting \ac{sn}~\cite{liu2020simple,van2021improving}, and thus preserving $L_2$ distances, typically fit \acp{gp} with RBF kernels on top of the learned feature space, extending distance awareness to the output layer.
%
In particular, SNGP~\cite{liu2020simple} relies on a Laplace approximation of the \ac{gp} based on the random Fourier feature (RFF) expansion of the \ac{gp} posterior~\cite{rasmussen2003gaussian}.
%
DUE~\cite{van2021improving} leverages instead the inducing point approximation~\cite{titsias2009variational,hensman2015scalable}, allowing to pick an arbitrarily large number of inducing points without overfitting~\cite{burt2019rates}.
%
%In practice, our experiments show that the RFF approximation allows for much more stable optimization, while still providing an excellent approximation of the posterior.
%
The uncertainty is then derived respectively as the Dempster-Shafer metric~\cite{liu2020simple} or the softmax entropy~\cite{van2021improving}.
%

% While some of the uncertainty models are ideal for a specific latent regularization strategy, \eg{} \acp{gp} with RBF kernels benefit from spectral normalized networks~\cite{liu2020simple}, in principle all models can be applied to the feature space encoded with any of the previously introduced techniques.

%
%Preliminary approaches attempted to model densities in the feature space of discriminative models under Gaussian discriminant analysis~\cite{lee2018simple}. Since it does not address feature collapse, this method occasionally fails to separate in-distribution from OOD data. 
%

%

%Alemi \etal~\cite{alemi2018uncertainty} fit a Gaussian Mixture Model (GMM) on the variational information bottleneck (VIB). 
%

%the full posterior over parameter space, allowing to quantify uncertainty in a single forward pass thanks to the modelling of the density of the features~\cite{ardizzone2018analyzing,nalisnick2019hybrid,ardizzone2020training} typically done through normalizing flows.



==> sections_old/4_1_image_classification.tex <==
\textbf{Datasets.} 
%
We train \acp{dum} on MNIST~\cite{lecun1998mnist}, FashionMNIST~\cite{xiao2017fashion}), CIFAR-10~\cite{krizhevsky2014cifar} and SVHN~\cite{netzer2011reading}). 
%
Further, when evaluating \ac{ood} detection, we also evaluate on Omniglot~\cite{lake2015human} for models trained on MNIST/FashionMNIST and on STL-10~\cite{coates2011analysis} for models trained on CIFAR10/SVHN.
%

\textbf{Models and optimization.} 
%
For the experiments on MNIST and Fashion-MNIST, we employ a \ac{mlp} as feature extractor with $3$ hidden layers of $100$ dimensions each and ReLU activation functions.
%
When training on CIFAR-10 and SVHN, we use a ResNet-18~\cite{he2016deep} as backbone.
%
Each \ac{dum} is associated with a particular hyperparameter for the regularization of its hidden representations. We choose the hyperparameter such that it minimizes the validation loss in the experiments on \ac{ood} detection and calibration. However, this section also includes an analysis of the sensitivity of calibration and \ac{ood} detection performance to the hyparameter (\autoref{fig:sensitivity_to_regularization_strength}).
%
All results are averages  $5$ distinct trainings.
%
We refer to the supplement for a detailed description on the optimization procedure for each \ac{dum}.

\textbf{Continuous distributional shifts.} 
%
We evaluate calibration of \acp{dum} on continuously shifted test data. Therefore, we apply rotations to MNIST/FashionMNIST in steps of $20\degree$ from $0\degree$ to $180\degree$. When evaluating on SVHN/CIFAR10 we add Gaussian noise of increasing standard deviation $\sigma$ to the test data. We vary $\sigma$ in steps of $0.05$ from $0$ to $0.25$ (on normalized data).
%

\subsubsection{Results} \label{ssec:classification_results}

\textbf{Calibration under continuous distributional shift.} \autoref{tab:classification_cal} shows accuracy on the test set and calibration performance in terms of \ac{raulc}. With the exception of DUQ, which we find to be prone to training instabilities, all \acp{dum} achieve similar predictive performance as \ac{mc} dropout, deep ensembles and standard softmax models. In terms of uncertainty calibration, we observe that in particular DUE, SNGP and MIR compete with established uncertainty estimation methods (\eg{} \ac{mc} dropout) across most datasets and both types of distributional shifts. Consequently, these approaches do not only fare well at detecting \ac{ood} data but also deliver well calibrated uncertainties under synthetic distributional shifts.
%
However, this is not sufficient to justify their use for real-world safety-critical applications.
%
Refer to \autoref{ssec:segmentation_results} for an analysis of calibration under realistic distributional shift.
% making them strong candidates for application in scenarios where both uncertainty and fast inference are imperative.

\begin{figure*}[t]
\begin{tabular}{ccc}

\multicolumn{3}{c}{\input{figures/image_classification/acc_aulc_auroc_vs_perturbation/custom_legend}}
\\

\input{figures/image_classification/acc_aulc_auroc_vs_perturbation/mnist_ACC_vs_perturbation} &
\input{figures/image_classification/acc_aulc_auroc_vs_perturbation/mnist_AUROC_vs_perturbation} &
\input{figures/image_classification/acc_aulc_auroc_vs_perturbation/mnist_AULC_vs_perturbation}
\\

\input{figures/image_classification/acc_aulc_auroc_vs_perturbation/svhn_ACC_vs_perturbation} &
\input{figures/image_classification/acc_aulc_auroc_vs_perturbation/svhn_AUROC_vs_perturbation} &
\input{figures/image_classification/acc_aulc_auroc_vs_perturbation/svhn_AULC_vs_perturbation}

\end{tabular}
\vspace{-1em}
\caption{We compare \acp{dum} and the baselines (\ac{mc} dropout (MCD), ensembles (Ens)) under continuous distributional shifts. Therefore, we plot accuracy (LEFT), \ac{auroc} (CENTER) and \ac{raulc} (RIGHT) against the perturbation magnitude for a MLP trained on MNIST (TOP) and a ResNet-18 on SVHN (BOTTOM). We perturbe MNIST using rotations and SVHN using additive Gaussian noise. The \ac{auroc} is computed against unperturbed test data. Most \acp{dum} demonstrate similar behaviour as the baselines, except DDU. While MIR shows strong performance on MNIST, its performance drops on CIFAR10.}\label{fig:acc_aulc_auroc_vs_perturbation}
\end{figure*}


\begin{table}[t]
\small
    \centering
    \setlength{\tabcolsep}{2.8pt}
    \input{tables/classification_cal}
    \caption{We evaluate the in-domain test accuracy (Acc, \%) and calibration performance (\ac{raulc}, \%) on MNIST, FashionMNIST, CIFAR10 and SVHN datasets. The backbones for all methods are MLP for MNIST/FashionMNIST and ResNet-18 for CIFAR10/SVHN. We observe that - in particular - DUE, SNGP and MIR are well calibrated across several scenarios.}
    \label{tab:classification_cal}
\end{table}

\begin{table}[t]
\small
    \centering
    \setlength{\tabcolsep}{3pt}
    \input{tables/classification_ood}
    \caption{Experiments for OOD detection (AUROC and AUPR, \%). The baseline method and all \acp{dum} use a MLP trained on MNIST/FashionMNIST and predict on another dataset. MIR demonstrates strong performance. (F-MNIST $=$ FashionMNIST).}
    \label{tab:classification_ood1}
\end{table}

\textbf{\ac{ood} Detection.} \autoref{tab:classification_ood1} shows quantitative results on detecting \ac{ood} data for \acp{dum}, \ac{mc} dropout, softmax entropy and deep ensembles trained on MNIST/FashionMNIST (similarly in the supplement for ResNet-18 trained on CIFAR10/SVHN). Among \acp{dum}, SNGP and MIR demonstrate the best performance across a variety of scenarios. While \acp{dum} confirm to be naturally suited for \ac{ood} detection, other established approaches (\eg{} \ac{mc} dropout) remain competitive. We note a particular drop in performance for \acp{dum} estimating uncertainty based on the distribution of hidden representations (\ie MIR and DDU) in the case of CIFAR10 vs. SVHN (see supplement). We hypothesize that this results from difficulties of generative models at distinguishing CIFAR10 and SVHN \cite{nalisnick2018deep}.
%
% \vspace{-1em}

% \begin{table}[htbp]
% \small
%     \centering
%     \setlength{\tabcolsep}{3pt}
%     \input{tables/classification_ood_2}
%     \caption{Experiments for OOD detection's performance (AUROC and AUPR, \%). The baselines and all \acp{dum} use a ResNet-18 trained on CIFAR10/SVHN and predict on another dataset.}
%     \label{tab:classification_ood2}
% \end{table}

\textbf{Sensitivity to Regularization Strength.} The hyperparameter associated with each \ac{dum} constitutes an important element in each method. It is important to know whether their performance in terms of \ac{ood} detection and calibration is sensitive to its choice. Intuitively, we expect the regularization technique to be positively correlated with \ac{ood} detection performance, since this is what most \acp{dum} were designed for. For each regularization paradigm - distance-awareness (SNGP) and informative representations (MIR) -, \autoref{fig:sensitivity_to_regularization_strength} visualizes the calibration (\ac{raulc}) and \ac{ood} detection (\ac{auroc}) performance depending on the strength of the regularization (similarly for other datasets and methods in the supplement). Most interestingly, we find that \acp{dum} regularizing the Lipschitz constant of the underlying feature extractor do not show evidence for a correlation between the regularization strength and the performance on \ac{ood} detection. One possible reason for this result is that Lipschitz-regularization is defined in the context of a particular predefined norm (\eg{} $L_2$) (see \autoref{sec:taxonomy}). However, this norm does not necessarily represent meaningful distances on a particular dataset (\eg{} images). On the contrary, in the case of enforcing informative representations using reconstruction regularization (MIR), we find evidence for a correlation between regularization strength and performance in terms of both \ac{ood} detection and calibration.


\begin{figure}[t]
\begin{tabular}{ccc}
\vspace{-4mm}
\input{figures/image_classification/regularization_strength_error_bars/mir_mnist_AULC_vs_ACC} & 
\input{figures/image_classification/regularization_strength_error_bars/mir_mnist_fashion_mnist_AUROC_vs_ACC} &
\input{figures/image_classification/regularization_strength_error_bars/mir_mnist_omniglot_AUROC_vs_ACC} 
\\ \vspace{-1mm}
\input{figures/image_classification/regularization_strength_error_bars/sngp_mnist_AULC_vs_ACC} & 
\input{figures/image_classification/regularization_strength_error_bars/sngp_mnist_fashion_mnist_AUROC_vs_ACC} & \hspace{-3mm}
\input{figures/image_classification/regularization_strength_error_bars/sngp_mnist_omniglot_AUROC_vs_ACC}
% \input{figures/image_classification/regularization_strength_error_bars/duq_mnist_AULC_vs_ACC} & 
% \input{figures/image_classification/regularization_strength_error_bars/duq_mnist_fashion_mnist_AUROC_vs_ACC} &
% \input{figures/image_classification/regularization_strength_error_bars/duq_mnist_omniglot_AUROC_vs_ACC} 
% \\
\end{tabular}
\vspace{-0.5em}
\caption{Trained on MNIST. Vertical axis: Test accuracy. Horizontal axis: \ac{raulc} (left), \ac{auroc} against FashionMNIST (center) and Omniglot (right) for MIR (top) and SNGP (bottom) using different regularization strength. For SNGP a larger hyperparameter corresponds to less regularization. For MIR we observe a correlation between regularization strength and performance.}\label{fig:sensitivity_to_regularization_strength}
\vspace{-1em}
\end{figure}

==> sections_old/4_2_large_scale_visual_task.tex <==
% \textcolor{cyan}{From Tao: Should we discuss the distinction of the dense prediction tasks here? 
% \begin{enumerate}
%     \item Pixel independence. We consider the pixel-level uncertainty and take each pixel independently (e.g. SNGP). Does this makes a difference than. each pixel is considered as a different classification problem
%     \item Realistic shift. We evaluate our models in a more realistic OOD shift, rather than synthetic shift (e.g. Gaussian blur, rotation). 
% \end{enumerate}
% }
%

\acp{dum} have been particularly motivated by prior work from a practical perspective due to their fast inference speed. 
% 
However, no practical extension of such methods to dense prediction tasks has been proposed yet.
%
This section evaluates whether \acp{dum} seamlessly scale to realistic vision tasks and compares their behaviour under realistic, continuous distributional shifts with \ac{mc} dropout. Therefore, we choose MIR~\cite{postels2020hidden} and SNGP~\cite{liu2020simple}, which both demonstrate good performance on uncertainty estimation for image classification and utilize conceptually different underlying regularization techniques, and adapt them to semantic segmentation.

We consider semantic segmentation as a multidimensional classification problem, where for each pixel of the output mask represents an independent classification problem. 
%
Given an image $\bfx$ with $n$ pixels $\bfy = \{y_1, \cdots, y_n\}$, the predictive distribution factorizes according to
%
$p(\bfy \mid \bfx) = p(y_1 \mid \bfx) p(y_2 \mid \bfx) \cdots p(y_n \mid \bfx)$.
%
% \begin{equation}
%     p(\bfy \mid \bfx) = p(y_1 \mid \bfx) p(y_2 \mid \bfx) \cdots p(y_n \mid \bfx)
% \end{equation}
%
We are interested in a global uncertainty estimate for the output map as our distributional shifts act on a global scale (see \autoref{ssec:segmentation_dataset}) and, thus, use the average pixel-level uncertainty as an image-level uncertainty.
%
% Consequently, we can easily extend each deterministic uncertainty method by simply estimating each per-pixel output density conditioned on the last feature space, and by treating each pixel as an independent classification problem.
%
% Since we want to estimate a global uncertainty estimate for the output map and we are not interested in pixel-level confidence, we propose to approximate the uncertainty of the predicted segmentation masks as the average of all pixel-level uncertainties.
%

While for image classification we simulated domain shift through synthetic distributional shifts, \ie{} additive Gaussian noise and rotation, for semantic segmentation we are interested in challenging current methods with realistic continuous distributional shifts along natural directions. \autoref{ssec:segmentation_dataset} describes the dataset we collected for this purpose.
%
In \autoref{ssec:segmentation_method_details} we report architectural choices and we detail how we extended the chosen \acp{dum} to dense prediction tasks. 
%
Results and findings are discussed in \autoref{ssec:segmentation_results}.

% To this end, we collect a synthetic dataset from the CARLA simulator, which allows to manipulate domain shift along natural directions, \eg{} brightness, weather conditions, azimuth angle of the sun...

%
%
\subsubsection{Dataset} \label{ssec:segmentation_dataset}
To benchmark our model in a realistically and continuously changing environment, we collect a synthetic dataset for semantic segmentation. 
%
We use the CARLA Simulator~\cite{Dosovitskiy17} for rendering the images and segmentation masks. The classes definition is aligned with the CityScape dataset~\cite{Cordts2016Cityscapes}. 
% In order to obtain a fair comparison, all the OOD data are sampled with the same trajectory and the environmental objects, except for the time-of-the-day or weather parameters. 

\textbf{Training data.} Data is collected from four towns in CARLA. We produce 32 sequences from each town. Vehicles and pedestrians are randomly generated for each sequence. Every sequence has 500 frames with a sampling rate of $10$ FPS. We uniformly sample a validation set.

\textbf{Continuous Distributional Shifts.} We use the time-of-the-day (weather conditions in the supplement) as the parameter for continuously changing the distribution. Visual examples and details on data collection are in the appendix. The time-of-the-day is parametrized by the Sun's altitude angle, where $90^\circ$ means the mid-day (training data) and the $0^\circ$ means the dust/dawn. We produce samples with altitude angles from $90^\circ$ to $15^\circ$ by steps of $5^\circ$, and $15^\circ$ to $-5^\circ$, where the environment changes sharply, in $1^\circ$ steps.
%
\subsubsection{Method Details} \label{ssec:segmentation_method_details}
\textbf{Backbone.} 
%
We adopt \ac{drn}~\cite{Yu2016, Yu2017} as semantic segmentation backbone. 
%
\ac{drn} introduces dilated convolutions to ResNet, effectively increasing the receptive field without increasing the number of layers or parameters. This improves the spatial accuracy of \ac{drn}, achieving satisfactory results on CityScapes~\cite{Cordts2016Cityscapes}. 
%
We adopt the variant DRN-A-50.
%
% (ablation in supplement).
%
All experiments were run $3$ times.
% for all the experiments.

\textbf{SNGP.} 
%
\ac{drn} uses $1 \times 1$ convolutions at the last layer to map the latest feature map to the predicted segmentation mask.
%
This works under the assumption that all pixels in the output mask are i.i.d. random variables.
%
Following this intuition, we extend SNGP to semantic segmentation by fitting a $GP: \mathbb{R}^Z \rightarrow \mathbb{R}^C$  at pixel level that maps from the deep feature dimension $z$ to the number of classes $c$. By keeping the \ac{gp} kernel parameters shared across all pixels, we simulate a  $1 \times 1$ convolutional \acp{gp}, \ie{} $\sigma: (H_l \times W_l \times Z) \rightarrow (H_l \times W_l \times C)$, where $\sigma$ convolves the \ac{gp}, $H_l$ and $W_l$ are respectively feature map height and width at layer $l$, $Z$ is the number of latent features and $C$ is the number of output classes. For details about the \ac{gp} we refer to \cite{liu2020simple} or the supplement.
%

\textbf{MIR.} To estimate image-level uncertainty MIR requires fitting the distribution of hidden representations. We fit a \ac{gmm} with $20$ components (\ie{} number of classes) to each spatial location of the hidden representations using features extracted from the training data independently. This assumes that the distribution is translation invariant and factorizes along the spatial dimensions of the latent space which is similar to the procedure used in \cite{blum2019fishyscapes}. We refer to the supplement for more details and computation of pixel-level uncertainties in this framework.

\subsubsection{Results} \label{ssec:segmentation_results}
\textbf{Continuous Distribution Shift.} 
%
We compare \acp{dum} with \ac{mc} dropout and the softmax baseline.
%
in terms of their calibration under realistic distributional shifts.
%
\autoref{table:calibration_segmentation} shows quantitative results. Encouragingly, all methods yield similar performance in terms of \ac{miou} and pixel accuracy. However, we observe that while \acp{dum} yield a considerable improvement over the softmax entropy - both in \ac{ood} detection and calibration - using a similar computational budget, these methods still fall short of established approaches, such as \ac{mc} dropout, in terms of calibration under challenging realistic distributional shifts. 
%
This finding is further supported by the results of \autoref{fig:miou_auroc_lc}, which shows 
%
% the \ac{miou}, \ac{auroc} and \ac{raulc} against the distributional shift. 
%
that \acp{dum} behave poorly in terms of calibration (see Lift curves) under realistic distributional shift.
%
We believe that these shortcomings must be addressed before practical deployment.


\begin{table}[t]
    \centering
    \scalebox{0.9}{
    \input{tables/segmentation}
    }
    \caption{We compare predictive performance on unperturbed test data - pixel accuracy (Acc.) and \ac{miou} - and calibration (rAULC) on realistic continuous distributional shifts of softmax, \ac{mc} dropout (MCD), SNGP and MIR on semantic segmentation. While SNGP and MIR perform better than the simple softmax baseline, they remain outclassed by \ac{mc} dropout in terms of calibration.}
    \label{table:calibration_segmentation}
    \vspace{-1em}
\end{table}

\begin{figure}

\begin{tabular}{ccc}

\multicolumn{3}{c}{\input{figures/semantic_segmentation/custom_legend}}
\\

\input{figures/semantic_segmentation/segmentation_mIoU_vs_perturbation} &
\input{figures/semantic_segmentation/segmentation_AUROC_vs_perturbation} &
\input{figures/semantic_segmentation/segmentation_LC_summary}

\end{tabular}
\caption{We compare the \ac{miou} (left), \ac{auroc} (center) and \ac{raulc} (right) of softmax (SM), \ac{mc} dropout (MCD), SNGP and MIR under realistic continuous distributional shifts. The \ac{auroc} is computed against unperturbed test data. While the softmax entropy as a measure of uncertainty clearly fails in this scenario, \acp{dum} (SNGP/MIR) yield reasonable uncertainty using a similar computational budget at identical predictive performance (\ac{miou}). However, \ac{mc} dropout, with its larger computational footprint, provides better calibrated uncertainty estimates (Lift).}\label{fig:miou_auroc_lc}
\vspace{-4mm}
\end{figure}


==> sections_old/4_experiments.tex <==
%
%The research effort on deterministic epistemic uncertainty modelling has so far focused on providing excellent confidence measure to detect \ac{ood} samples.
%
%However, the calibration of such epistemic uncertainty estimates is ambiguous close to the training distribution and is typically not assessed.
%
%Since discriminative models are often overconfident about the model's predictions~\cite{guo2017calibration,hein2019relu}, we argue that calibration of confidence measures is an indispensable property for practical use of such methods.

% Furthermore, while most of the proposed methods claim to be easily extendable to more complicated tasks and architectures, this has not been shown in practice. 
%
% In~\autoref{ssec:segmentation}, we successfully propose extended versions of some of these methods that scale to more challenging settings and outperform more popular and less efficient baselines. 
%
% Further, we evaluate how such techniques hold their promises on harder tasks, \eg semantic segmentation,  scaling nicely to the deeper architectures while providing inexpensive uncertainty estimates.
 %In this section, we introduce our setting for a complete and fair evaluation of \acp{dum}. 
 %
 We first benchmark \acp{dum} on popular image classification datasets (\autoref{ssec:classification}).
 %
 Further, we evaluate how such techniques scale to harder tasks, \eg{} semantic segmentation, by extending the most promising \acp{dum} to dense prediction tasks (\autoref{ssec:segmentation}).
 %
 Finally, in \autoref{ssec:segmentation_results} we find that uncertainty from the current generation of \acp{dum} is considerably worse calibrated under realistic distributional shift than scalable approaches based on stochastic regularization, \ie MC dropout.
%
% In both settings, we analyze their \ac{ood} detection performance and calibration compared to traditional deep uncertainty estimation baselines.

\textbf{Baselines.} We compare \acp{dum} with two established baselines for estimating epistemic uncertainty on image classification (\autoref{ssec:classification}) - \ac{mc} dropout \cite{gal2016dropout} and deep ensembles \cite{lakshminarayanan2017simple}. On semantic segmentation (\autoref{ssec:segmentation}) we compare only against \ac{mc} dropout since maintaining several set of weights of a large \ac{nn} dramatically increases memory requirements.
%
Note, that while these baselines are expected to predict reasonable uncertainty, their computational footprint greatly outweighs \acp{dum}. We also report the performance of the softmax entropy as a baseline deterministic uncertainty method.

\textbf{Methods.} For this comparison, we choose \acp{dum} according to their potential to benefit real-world applications. 
%
We thus value \acp{dum} that can readily scale to large vision tasks (\eg{} semantic segmentation). Therefore, we exclude \acp{dum} that regularize hidden representations using contrastive learning~\cite{wu2020simple}, which requires very large batch sizes and long training times, and invertible neural networks \cite{nalisnick2019hybrid, ardizzone2020training}, which enforce strict constraints on the underlying architecture (\eg{} fixed dimensionality of hidden representations) and often lead to training instabilities. 
%
Moreover, we do not include DCS~\cite{mandelbaum2017distance}
since it only leads to a marginal improvement over the softmax entropy according to their own experiments, and since their contrastive loss only operates on class centroids and, thus, is not expected to lead to distance awareness within clusters. 
%
% used to achieve effective embeddings 
%

% Thus, for the experiments on image classification \autoref{ssec:classification} we choose representative methods for each category of the proposed taxonomy \autoref{sec:taxonomy}: DUQ~\cite{van2020uncertainty}, SNGP~\cite{liu2020simple}, and DUE~\cite{van2021improving} using distance-aware hidden representations and discriminative uncertainty estimation; DDU~\cite{mukhoti2021deterministic} as the only method with distance-aware embeddings and generative uncertainty estimation; and MIR~\cite{postels2020hidden} using generative uncertainty estimation and enforcing informative representations. According to \autoref{table:taxonomy}, to the best of our knowledge no discriminative model from informative representations has been proposed yet.
%
%

% \textbf{talk about which models are scaled to semantic segmentation.}
% Finally, we
% \cite{van2020uncertainty, liu2020simple, van2021improving, mukhoti2021deterministic, postels2020hidden}

\textbf{\ac{ood} detection metrics.} 
%
We follow prior work~\cite{liu2020simple, postels2020hidden} and compute \ac{auroc} and \ac{aupr} between test data that originates from the same distribution as the training data and data originating from another dataset (\autoref{ssec:classification_results}). 

\textbf{Calibration metric.} 
%
% For measuring the calibration of epistemic uncertainty under continuous distributional shifts, it is necessary to introduce a novel metric.
%
In order to assess the calibration of uncertainty estimates under distributional shifts, we need to introduce a novel metric, since \ac{ece} \cite{naeini2015obtaining} and Brier score \cite{brier1950verification}  are limited to probabilistic forecasts (\ie{} methods producing calibrated probabilities).
% , when 
% assessing the calibration of \acp{dum} this evaluation scheme
% evaluating \acp{dum} this is 
%and thus not directly applicable to deterministic approaches that approximate uncertainty as the log-likelihood of hidden representations (\eg{} \cite{postels2020hidden, wu2020simple, mukhoti2021deterministic}) or distances in the latent space \cite{mandelbaum2017distance, van2020uncertainty}. 
%
% These approaches yield a - potentially uncalibrated - predictive distribution and an uncertainty quantifying the trustworthiness of the prediction. 
%
% In order to assess how well estimated uncertainty is calibrated under distributional shifts, we use the \ac{aulc} \cite{vuk2006roc}. 
%
%Based on the intuition that a well calibrated uncertainty score should be a good indicator for expected model performance, we propose to measure how well an uncertainty score performs at ordering the samples according to the predictive performance of a discriminative model on continuously shifted data.
%
Therefore, we calculate the \ac{aulc}~\cite{vuk2006roc}, which we obtain by ordering the predictions according to increasing uncertainty and plotting the performance (\eg{} accuracy) of all samples with an uncertainty estimate smaller than a certain quantile of the uncertainty against the quantile of uncertainty. 
%
Formally, given a set of uncertainty quantiles $q_i \in [0, 1]$, $i\in [1, ..., N]$, with some quantile step width $0<s<1$
%
% where $i\in [1, ..., N]$ 
%
and the function $F(q_i)$ which returns the accuracy of all samples with uncertainty $u < q_i$, we define the \ac{aulc} as $AULC =  - 1 + \sum_{i\in [1, ..., N]} s \frac{F(q_i)}{F_R(q_i)}$. Here, $F_R(\cdot)$ refers to a baseline uncertainty estimate that corresponds to random guessing, and we subtract 1 to shift the performance of the random baseline to zero.
%
Note, if an uncertainty estimate is anti-correlated with a models' performance, this score can also be negative. 
%
To alleviate bias towards better performing models, we further compute the \ac{raulc} by dividing the \ac{aulc} by the \ac{aulc} of a hypothetical (optimal) uncertainty estimation that perfectly orders samples according to model performance. In classification samples are ordered according to correct/incorrect prediction. In semantic segmentation we use the image-level pixel accuracy. 

\subsection{Image Classification}\label{ssec:classification}
\input{sections/4_1_image_classification}


\subsection{Semantic Segmentation}\label{ssec:segmentation}
\input{sections/4_2_large_scale_visual_task}


==> sections_old/5_conclusion.tex <==
%
While \acp{dum} show good \ac{ood} detection performance and are interesting for practical applications in need of efficient uncertainty quantification, we find them struggling regarding calibration under realistic distributional shifts. 
%
Despite promising results of uncertainty on toy datasets, this does not extrapolate to more realistic scenarios (\autoref{ssec:segmentation}). 
%
We find that, while \acp{dum} outperform the softmax entropy, \ac{mc} dropout clearly outperforms \acp{dum} regarding uncertainty calibration.

Moreover, another desirable property for such methods would be that the strength of the feature space regularization correlates with the quality of \ac{ood} detection. 
%
% In particular, being distance awareness the aim of Lipschitz regularization, one might expect that \ac{ood} detection performance correlates well with regularization strength.
% for methods relying on gradient penalty or spectral normalization to regularize the feature space. 
%
However, this is not verified for Lipschitz regularization by our investigation. We hypothesize that this originates from the choice of metric for regularization - \ie{} $L_2$ distance - which is not meaningful in the image space.
%
% As expected, the lack of correlation also extends to calibration performance. 
% regularization parameters, highlighting how current proposals cannot be reliably deployed under distributional shift as a proxy for risk-informative decision-making in safety-critical applications.
We hope that our findings will foster future research on making these promising family of methods better calibrated and more broadly applicable.

% \mattia{
% say that we expect the strength of regularization to correlate well with the performance on ood detection, since the regularization techniques are specifically designed for that. While such regularization techniques are actually effective for ood detection, making unclear whether the regularization technique actually helps. also say that we expect it may not be because of the choice of the norm. in sectiono we validate our findings
% how to choose hyperparameter for dums? since we cannot tune them on ood data, simply choosing them to maximise the model accuracy may not correlate well with ood detection performance. there is no clear way to choose this param
% no theoretical evidence of correlation of tuning of this parameter and calibration, maybe there is for ood detection}

==> tables/classification_cal.tex <==
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\multirow{2}{*}{{Method}} & \multicolumn{2}{c}{\textbf{MNIST}}   & \multicolumn{2}{c}{\textbf{FashionMNIST}} & \multicolumn{2}{c}{\textbf{CIFAR10}} & \multicolumn{2}{c}{\textbf{SVHN}}    \\ \cmidrule(l){2-3}  \cmidrule(l){4-5} \cmidrule(l){6-7} \cmidrule(l){8-9}
                        & Acc          & \ac{raulc}         & Acc             & \ac{raulc}           & Acc          & \ac{raulc}         & Acc          & \ac{raulc}         \\ \midrule
Softmax                 & {98.1 $\pm$ 0.1} & 54.1 $\pm$ 3.4 & 88.1 $\pm$ 0.2    & 7.1 $\pm$ 2.9   & 84.5 $\pm$ 0.2 & 43.4 $\pm$ 17.4 & 93.2 $\pm$ 0.2 & 84.2 $\pm$ 0.5 \\
Dropout                 & 97.2 $\pm$ 0.1 & 59.2 $\pm$ 0.8 & 87.8 $\pm$ 0.2    & \textbf{48.4 $\pm$ 1.2}   & \underline{86.0 $\pm$ 0.2}  & \textbf{65.5 $\pm$ 0.8} & 94.0 $\pm$ 0.1  & 82.2 $\pm$ 0.1 \\
Ensemble                 & \textbf{98.6 $\pm$ 0.2} & 59.4 $\pm$ 1.4 & \underline{88.9 $\pm$ 0.2 }   & 24.3 $\pm$ 1.5   & \textbf{88.9 $\pm$ 0.2}  & {60.6 $\pm$ 3.2} & \textbf{95.2 $\pm$ 0.2}  & \underline{84.7 $\pm$ 1.4} \\ \midrule
DUE                     & \underline{98.1 $\pm$ 0.1} & 59.0 $\pm$ 2.0   & 88.6 $\pm$ 0.2    & 24.5 $\pm$ 3.1   & 84.6 $\pm$ 1.9 & 59.6 $\pm$ 3.2 & 88.5 $\pm$ 7.8 & 81.6 $\pm$ 4.5 \\
DUQ                     & 96.9 $\pm$ 0.1 & \underline{61.4 $\pm$ 1.2} & 87.4 $\pm$ 0.4    & 41.8 $\pm$ 1.5   & 77.2 $\pm$ 0.9 & 37.2 $\pm$ 13.2 & 91.5 $\pm$ 0.3 & 79.2 $\pm$ 3.4 \\
DDU                     & \underline{98.1 $\pm$ 0.1} & 38.3 $\pm$ 9.0  & \textbf{89.3 $\pm$ 0.1}   & 33.5 $\pm$ 9.7   & {85.5 $\pm$ 0.2} & 34.3 $\pm$ 10.9 & \underline{94.8 $\pm$ 0.2} & 67.7 $\pm$ 7.3 \\
SNGP                    & 97.7 $\pm$ 0.4 & 58.9 $\pm$ 4.6 & 86.4 $\pm$ 1.4    & 34.7 $\pm$ 3.7   & {85.5 $\pm$ 0.3} & \underline{64.6 $\pm$ 3.0}  & 94.0 $\pm$ 0.2  & \textbf{84.5 $\pm$ 0.6} \\
MIR                     & 97.6 $\pm$ 0.2 & \textbf{72.4 $\pm$ 1.1} & 87.4 $\pm$ 0.3    & \underline{47.4 $\pm$ 3.7}   & 85.3 $\pm$ 0.2 & 55.0 $\pm$ 5.7  & 94.1 $\pm$ 0.2 & 71.9 $\pm$ 3.1 \\
% VMIR                    & 96.6 $\pm$ 0.2 & 60.9 $\pm$ 2.6 & 86.6 $\pm$ 0.6    & 42.6 $\pm$ 5.2   & -            & -            & -            & -            \\ 
\bottomrule
\end{tabular}

==> tables/classification_ood.tex <==
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{\textbf{MNIST $\rightarrow$ F-MNIST}} & \multicolumn{2}{c}{\textbf{MNIST $\rightarrow$ Omniglot}} & \multicolumn{2}{c}{\textbf{F-MNIST $\rightarrow$ MNIST}} & \multicolumn{2}{c}{\textbf{F-MNIST $\rightarrow$ Omniglot}} \\ \cmidrule(l){2-3}  \cmidrule(l){4-5} \cmidrule(l){6-7} \cmidrule(l){8-9}
                        & AUROC                  & AUPR                   & AUROC                   & AUPR                   & AUROC                  & AUPR                   & AUROC                    & AUPR                    \\ \midrule
Softmax                 & 89.0 $\pm$ 1.2            & 88.5 $\pm$ 1.4           & \underline{95.1 $\pm$ 0.3}            & 94.5 $\pm$ 0.4           & 73.2 $\pm$ 3.5           & 75.9 $\pm$ 2.6           & 75.9 $\pm$ 1.5             & 74.1 $\pm$ 1.6            \\
Dropout                 & 94.4 $\pm$ 0.9          & 92.0 $\pm$ 1.8            & 94.8 $\pm$ 0.2            & 92.0 $\pm$ 0.5            & \underline{95.8 $\pm$ 0.2}           & 93.6 $\pm$ 0.6           & \underline{96.3 $\pm$ 0.2}             & \underline{94.3 $\pm$ 0.3}            \\
Ensemble                 & \underline{95.2$\pm$ 1.0}          & 91.4 $\pm$ 3.6            & \textbf{97.3 $\pm$ 0.4}            & \underline{95.3 $\pm$ 0.1 }           & {87.0 $\pm$ 1.5}           & 81.4 $\pm$ 0.3           & 90.7 $\pm$ 1.1             & 87.6 $\pm$ 2.5            \\\midrule
DUE                     & 90.8 $\pm$ 2.3           & 90.9 $\pm$ 2.0            & 94.2 $\pm$ 0.2            & 92.8 $\pm$ 0.2           & 68.2 $\pm$ 1.9           & 65.7 $\pm$ 3.0            & 72.4 $\pm$ 1.7             & 65.8 $\pm$ 2.8            \\
DUQ                     & 90.2 $\pm$ 3.0            & 92.2 $\pm$ 2.4           & 93.8 $\pm$ 0.3            & 93.8 $\pm$ 0.4           & 95.1 $\pm$ 1.1           & \underline{95.9 $\pm$ 1.0}            & 94.7 $\pm$ 0.6             & \underline{94.3 $\pm$ 0.7}            \\
DDU                     & 83.9 $\pm$ 7.6           & 83.4 $\pm$ 7.9           & 75.2 $\pm$ 6.7            & 69.4 $\pm$ 9.5           & 90.8 $\pm$ 5.5           & 92.2 $\pm$ 4.8           & 90.6 $\pm$ 4.6             & 90.3 $\pm$ 4.6            \\
SNGP                    & 93.2 $\pm$ 1.2           & \underline{94.6 $\pm$ 1.3}           & 94.8 $\pm$ 0.7            & 93.9 $\pm$ 0.7           & 89.2 $\pm$ 1.1           & 87.9 $\pm$ 1.3           & 89.8 $\pm$ 1.7             & 85.5 $\pm$ 2.7            \\
MIR                     & \textbf{97.0 $\pm$ 0.7}            & \textbf{97.7 $\pm$ 0.5}           & \textbf{97.3 $\pm$ 0.6}            & \textbf{97.4 $\pm$ 0.5}          & \textbf{99.0 $\pm$ 0.3}            & \textbf{99.2 $\pm$ 0.2}           & \textbf{97.9 $\pm$ 0.2}             & \textbf{97.6 $\pm$ 0.4}            \\
% VMIR                    & 91.6 $\pm$ 2.7           & 92.2 $\pm$ 2.6           & 89.7 $\pm$ 1.9            & 89.3 $\pm$ 1.9           & 98.6 $\pm$ 0.5           & 98.8 $\pm$ 0.4           & 97.6 $\pm$ 1.0              & 97.4 $\pm$ 1.0            \\
\bottomrule
\end{tabular}


==> tables/classification_ood_2.tex <==
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\multirow{2}{*}{{Method}} & \multicolumn{2}{c}{\textbf{CIFAR10 $\rightarrow$ SVHN}} & \multicolumn{2}{c}{\textbf{CIFAR10 $\rightarrow$ STL10}} & \multicolumn{2}{c}{\textbf{SVHN $\rightarrow$ CIFAR10}} & \multicolumn{2}{c}{\textbf{SVHN $\rightarrow$ STL10}} \\ \cmidrule(l){2-3}  \cmidrule(l){4-5} \cmidrule(l){6-7} \cmidrule(l){8-9}
                        & AUROC                 & AUPR                  & AUROC                 & AUPR                 & AUROC                   & AUPR                   & AUROC                  & AUPR                   \\ \midrule
Softmax                 & 83.1 $\pm$ 1.0           & 77.2 $\pm$ 1.8          & 67.4 $\pm$ 1.3          & 71.5 $\pm$ 1.2         & 93.1 $\pm$ 0.5            & 97.5 $\pm$ 0.2           & 93.6 $\pm$ 0.6           & 98.1 $\pm$ 0.2           \\
Dropout                 & \underline{85.2 $\pm$ 0.9}          & 76.5 $\pm$ 1.2          & 68.7 $\pm$ 0.3          & 72.8 $\pm$ 0.5         & 94.3 $\pm$ 0.4            & \underline{98.0 $\pm$ 0.1}            & 94.7 $\pm$ 0.3           & \underline{98.5 $\pm$ 0.1}           \\
Ensemble                 & 79.8 $\pm$ 2.9          & \textbf{97.6 $\pm$ 1.7}            & \textbf{98.2 $\pm$ 1.8}            & 85.8 $\pm$ 3.4           & \textbf{99.3 $\pm$ 1.1}           & 97.7 $\pm$ 3.5           & \textbf{98.3 $\pm$ 0.5}            & 96.8 $\pm$ 2.3            \\\midrule
DUE                     & 84.3 $\pm$ 4.7          & 77.4 $\pm$ 7.3       & 71.3 $\pm$ 2.6          & 75.5 $\pm$ 3.0          & 92.2 $\pm$ 3.3            & 97.0 $\pm$ 1.4            & 92.4 $\pm$ 3.5           & 97.7 $\pm$ 1.2           \\
DUQ                     & 76.8 $\pm$ 5.0           & 67.2 $\pm$ 6.3          & 65.1 $\pm$ 1.9          & 70.8 $\pm$ 1.0          & 90.1 $\pm$ 1.2            & 96.3 $\pm$ 0.4           & 91.1 $\pm$ 1.5           & 97.3 $\pm$ 0.4           \\
DDU                     & 69.0 $\pm$ 6.3           & 51.1 $\pm$ 7.4          & 68.9 $\pm$ 3.6          & 72.8 $\pm$ 3.2         & 73.4 $\pm$ 5.5            & 89.8 $\pm$ 2.4           & 76.7 $\pm$ 5.4           & 92.5 $\pm$ 2.0            \\
SNGP                    & \textbf{85.3 $\pm$ 4.7}          & \underline{79.4 $\pm$ 6.5}          & \underline{76.1 $\pm$ 1.7}          & \underline{79.4 $\pm$ 1.5}         & \underline{95.8 $\pm$ 0.3}            & \textbf{98.4 $\pm$ 0.1}           & \underline{96.4 $\pm$ 0.3}           & \textbf{98.9 $\pm$ 0.1}           \\
MIR                     & 85.0 $\pm$ 6.0            & 71.4 $\pm$ 11.7          & 72.2 $\pm$ 2.1          & \underline{76.3 $\pm$ 2.0}          & 91.6 $\pm$ 1.2            & 97.0 $\pm$ 0.4            & 92.8 $\pm$ 1.2           & 97.9 $\pm$ 0.3     \\     
\bottomrule
\end{tabular}

==> tables/segmentation.tex <==
% \begin{tabular}{lccc}
% \toprule
% \multirow{2}{*}{Method} & \multicolumn{2}{c}{\textbf{In-domain Testset}} & \multicolumn{1}{c}{\textbf{Time-of-the-Day}} \\ 
% \cmidrule(l){2-3} \cmidrule(l){4-4}
%                         & Acc (\%)          & mIoU (\%)        & \ac{raulc} (\%)                             \\ 
%                         \midrule
% Softmax                 & 93.0 $\pm$ 0.1  & 44.3 $\pm$ 0.4 & 25.9 $\pm$ 3.1                        \\
% Dropout                 & 92.9 $\pm$ 0.1 & 44.0 $\pm$ 0.4  & \textbf{91.2 $\pm$ 1.2}                        \\
% SNGP                    & 93.2 $\pm$ 0.1 & 44.4 $\pm$ 0.0   & 66.7 $\pm$ 4.1                        \\
% MIR                     & 93.0 $\pm$ 0.1  & 44.2 $\pm$ 0.0   & \underline{72.5 $\pm$ 4.1}      \\
% \bottomrule
% \end{tabular}
\begin{tabular}{llcccc}
\toprule
\multicolumn{2}{l}{\textbf{Method}}      & Softmax      & MCD      & SNGP         & MIR          \\
\midrule
\multirow{2}{*}{\textbf{In-domain Testset}} & Acc (\%) & 93.0 $\pm$ 0.1  & 92.9 $\pm$ 0.1 & 93.2 $\pm$ 0.1 & 93.0 $\pm$ 0.1  \\
                         & mIoU (\%) & 44.3 $\pm$ 0.4 & 44.0 $\pm$ 0.4  & 44.4 $\pm$ 0.0   & 44.2 $\pm$ 0.0   \\
                         \cmidrule(l){2-6}
\textbf{Time-of-the-Day}         & rAULC & 25.9 $\pm$ 3.1 & \textbf{91.2 $\pm$ 1.2} & 66.7 $\pm$ 4.1 & \underline{72.5 $\pm$ 4.1} \\
\bottomrule
\end{tabular}

==> tables/segmentation2.tex <==
\begin{tabular}{llcccc}
\toprule
\multicolumn{2}{l}{\textbf{Method}}      & Softmax      & MC Dropout      & SNGP         & MIR          \\
\midrule
\multirow{2}{*}{\textbf{In-domain Testset}} & Acc (\%)  & 93.0 $\pm$ 0.1  & 92.9 $\pm$ 0.1 & 93.2 $\pm$ 0.1 & 93.0 $\pm$ 0.1  \\
\multicolumn{1}{c}{}                         & mIoU (\%) & 44.3 $\pm$ 0.4 & 44.0 $\pm$ 0.4  & 44.4 $\pm$ 0.0   & 44.2 $\pm$ 0.0   \\
\cmidrule(l){2-6}
\textbf{Weather Conditions}                              & RAULC ($\cdot 10^3$) & 70.8 $\pm$ 2.6 & \textbf{86.1 $\pm$ 0.5} & 81.3 $\pm$ 1.2 & \underline{72.6 $\pm$ 0.5} \\
\bottomrule
\end{tabular}

==> tables/taxonomy.tex <==
\begin{table}
  \caption{Taxonomy of \acp{dum}. Methods are grouped according to (i) the target property of the hidden representations and (ii) their uncertainty estimation method. Moreover, we name the regularization technique used to achieve (i).}
  \label{table:taxonomy}
  \centering
  \setlength{\aboverulesep}{0pt}
  \setlength{\belowrulesep}{0pt}
  \renewcommand{\arraystretch}{1.35}
  \scalebox{0.9}{
  \begin{tabular}{|l|l|l|l|}
    \hline
    \multicolumn{2}{|c|}{Feature Space Manipulation} & \multicolumn{2}{|c|}{Deterministic Uncertainty Methods} \\
    \hline
    Target Property                          & Strategy                 & Method       & Uncertainty Estimation  \\
    \hline
    \multirow{6}{*}{Distance Awareness}      & Adversarial Augmentation & \multirow{2}{*}{DCS~\cite{mandelbaum2017distance}} & Distance Confidence Score     \\ 
    \cline{2-2}\cline{4-4}
                                             & Supervised Contrastive Learning &  & Distance Confidence Score     \\            
    \cline{2-4}
                                             & Two-sided Gradient Penalty~\cite{gulrajani2017improved} & DUQ~\cite{van2020uncertainty}         & Distance from centroid     \\
    \cline{2-4}
                                             & \multirow{3}{*}{SN and Residual Connections} & SNGP~\cite{liu2020simple}        & RFF GP    \\
                                             &                                              & DUE~\cite{van2021improving}      & Inducing Points GP     \\
                                             &                                              & DDU~\cite{mukhoti2021deterministic}         & GMM \\
    \cline{1-4}
    \multirow{3}{*}{Informative Representations} & Variational Bottleneck                & VIB~\cite{alemi2018uncertainty} & GMM     \\
    \cline{2-4} 
                                                 & Contrastive Learning          & DCU~\cite{wu2020simple} & Distribution variance     \\
    \cline{2-4} 
                                                 & Reconstruction Regularization                & MIR~\cite{postels2020hidden} & GMM     \\
    \cline{2-4}
                                                 & Invertible Networks~\cite{jacobsen2018revnet,behrmann2018invertible} & ~\cite{ardizzone2018analyzing,nalisnick2019hybrid, ardizzone2020training}           & Normalizing Flows     \\
    \bottomrule
  \end{tabular}
  }
\end{table}

==> tables/taxonomy_v1.tex <==
\begin{table}
  \caption{Taxonomy of \acp{dum}. Methods are grouped according to: (i) the target property of the hidden representations and the regularization strategy used to achieve it; (ii) their uncertainty estimation method.}
  \label{table:taxonomy}
  \centering
  \setlength{\aboverulesep}{0pt}
  \setlength{\belowrulesep}{0pt}
  \renewcommand{\arraystretch}{1.35}
  \scalebox{0.9}{
  \begin{tabular}{|c|c|c|c|}
    \hline
    \multicolumn{2}{|c|}{Regularization of Hidden Representations} & \multicolumn{2}{|c|}{Deterministic Uncertainty Methods} \\
    \hline
    Target Property                          & Strategy                 & Method       & Uncertainty Estimation  \\
    \hline
    \multirow{6}{*}{Distance Awareness}      & Adversarial Augmentation & \multirow{2}{*}{DCS~\cite{mandelbaum2017distance}} & \multirow{3}{*}{Distance from class centroid}     \\ 
    \cline{2-2}
                                             & Supervised Contrastive Learning &  & \\            
    \cline{2-3}
                                             & Two-sided Gradient Penalty & DUQ~\cite{van2020uncertainty}         & \\
    \cline{2-4}
                                             & \multirow{3}{*}{SN and Residual Connections} & SNGP~\cite{liu2020simple}        & \multirow{2}{*}{Gaussian Process Approximations}    \\
    \cline{3-3}
                                             &                                              & DUE~\cite{van2021improving}      &  \\
    \cline{3-4}
                                             &                                              & DDU~\cite{mukhoti2021deterministic}         & \multirow{4}{*}{Gaussian Mixture Models} \\
    \cline{1-3}
    \multirow{3}{*}{Informative Representations} & Variational Bottleneck                & VIB~\cite{alemi2018uncertainty} & \\
    \cline{2-3} 
                                                 & Contrastive Learning          & DCU~\cite{wu2020simple} & \\
    \cline{2-3} 
                                                 & Reconstruction Regularization                & MIR~\cite{postels2020hidden} & \\
    \cline{2-4}
                                                 & Invertible Networks & ~\cite{ardizzone2018analyzing,nalisnick2019hybrid, ardizzone2020training}           & Normalizing Flows     \\
    \bottomrule
  \end{tabular}
  }
\end{table}

==> tables/taxonomy_v2.tex <==
\begin{table}
  \caption{Taxonomy of \acp{dum}. Methods are grouped according to (i) the target property of the hidden representations and (ii) their uncertainty estimation method. Moreover, we name the regularization technique used to achieve (i).}
  \label{table:taxonomy}
  \centering
  \setlength{\aboverulesep}{0pt}
  \setlength{\belowrulesep}{0pt}
  \renewcommand{\arraystretch}{1.35}
  \scalebox{0.9}{
  \begin{tabular}{|c|c|c|c|}
    \hline
    \multicolumn{4}{|c|}{Deterministic Uncertainty Methods} \\
    \hline
    Target Property                            & Uncertainty Estimation & Method  & Regularization Strategy                       \\
    \hline
    \multirow{6}{*}{Distance Awareness}      & \multirow{3}{*}{Distance from class centroid}  & \multirow{2}{*}{DCS~\cite{mandelbaum2017distance}}   & Adversarial Augmentation    \\ 
    \cline{4-4}
                                             &  & & Supervised Contrastive Learning  \\            
    \cline{3-4}
                                              & & DUQ~\cite{van2020uncertainty} & Two-sided Gradient Penalty        \\
    \cline{2-4}
                                             & \multirow{2}{*}{Gaussian Process Approximations} & SNGP~\cite{liu2020simple} & \multirow{3}{*}{SN and Residual Connections}            \\
    \cline{3-3}
                                             & & DUE~\cite{van2021improving}  &                                                   \\
    \cline{2-3}
                                                & \multirow{4}{*}{Gaussian Mixture Models} & DDU~\cite{mukhoti2021deterministic} &                                                    \\
    \cline{1-1} \cline{3-4}
    \multirow{3}{*}{Informative Representations}   & & VIB~\cite{alemi2018uncertainty} & Variational Bottleneck               \\
    \cline{3-4} 
                                                  & & DCU~\cite{wu2020simple} & Contrastive Learning         \\
    \cline{3-4} 
                                                   & & MIR~\cite{postels2020hidden} & Reconstruction Regularization               \\
    \cline{2-4}
                                                  & Normalizing Flows   & ~\cite{ardizzone2018analyzing,nalisnick2019hybrid, ardizzone2020training} & Invertible Networks    \\
    \bottomrule
  \end{tabular}
  }
\end{table}

==> tables/taxonomy_v3.tex <==
\begin{table}
  \caption{Taxonomy of \acp{dum}. Methods are grouped according to (i) the target property of the hidden representations and (ii) their uncertainty estimation method. Moreover, we name the regularization technique used to achieve (i).}
  \label{table:taxonomy}
  \centering
  \setlength{\aboverulesep}{0pt}
  \setlength{\belowrulesep}{0pt}
  \renewcommand{\arraystretch}{1.35}
  \scalebox{0.7}{
  \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    \multicolumn{2}{|c|}{\multirow{2}{*}{\acp{dum}}} & \multicolumn{4}{|c|}{Uncertainty Estimations} \\
    \cline{3-6}
    \multicolumn{2}{|c|}{} & \shortstack{Distance from\\ class centroid} & \shortstack{Gaussian Process\\ Approximations} & \shortstack{Gaussian Mixture\\ Models} & \shortstack{Normalizing\\ Flows} \\
    \cline{1-6}
    \multirow{10}{*}{\shortstack{Target\\ Property}}  & \multirow{6}{*}{\shortstack{Distance\\ Awareness}}      & DCS~\cite{mandelbaum2017distance}\\ Adversarial Augmentation\\ or\\ Supervised Contrastive Learning & & &   \\            
    \cline{3-4}
     &                                           & \shortstack{DUQ~\cite{van2020uncertainty}\\ Two-sided\\ Gradient Penalty}    & & &     \\
    \cline{3-6}
     &                                          & & \shortstack{SNGP~\cite{liu2020simple} \\ SN and\\ Residual Connections}     & &        \\
    \cline{3-3}
     &                                          & & \shortstack{DUE~\cite{van2021improving} \\ SN and\\ Residual Connections}    & &                                                \\
    \cline{2-3}
     &                                             & & & \shortstack{DDU~\cite{mukhoti2021deterministic}\\ SN and\\ Residual Connections}  &                                                    \\
    \cline{3-4}
     & \multirow{3}{*}{\shortstack{Informative \\ Representations}}   & & & \shortstack{VIB~\cite{alemi2018uncertainty}\\ Variational\\ Bottleneck} &               \\
    \cline{3-4} 
     &                                               & & & \shortstack{DCU~\cite{wu2020simple}\\ Contrastive\\ Learning} &         \\
    \cline{3-4} 
     &                                                & & & \shortstack{MIR~\cite{postels2020hidden}\\ Reconstruction\\ Regularization} &               \\
    \cline{3-4}
     &                                               &  & &   & ~\cite{ardizzone2018analyzing,nalisnick2019hybrid, ardizzone2020training} Invertible Networks    \\
    \bottomrule
  \end{tabular}
  }
\end{table}
